Optimization for Medical Image Segmentation: Theory and Practice when evaluating with Dice Score or Jaccard Index

In many medical imaging and classical computer vision tasks, the Dice score and Jaccard index are used to evaluate the segmentation performance. Despite the existence and great empirical success of metric-sensitive losses, i.e. relaxations of these metrics such as soft Dice, soft Jaccard and Lovasz-Softmax, many researchers still use per-pixel losses, such as (weighted) cross-entropy to train CNNs for segmentation. Therefore, the target metric is in many cases not directly optimized. We investigate from a theoretical perspective, the relation within the group of metric-sensitive loss functions and question the existence of an optimal weighting scheme for weighted cross-entropy to optimize the Dice score and Jaccard index at test time. We find that the Dice score and Jaccard index approximate each other relatively and absolutely, but we find no such approximation for a weighted Hamming similarity. For the Tversky loss, the approximation gets monotonically worse when deviating from the trivial weight setting where soft Tversky equals soft Dice. We verify these results empirically in an extensive validation on six medical segmentation tasks and can confirm that metric-sensitive losses are superior to cross-entropy based loss functions in case of evaluation with Dice Score or Jaccard Index. This further holds in a multi-class setting, and across different object sizes and foreground/background ratios. These results encourage a wider adoption of metric-sensitive loss functions for medical segmentation tasks where the performance measure of interest is the Dice score or Jaccard index.

==> TMI - Dice/L1L2fig/fig.tex <==
\begin{figure*}[htbp]%
% https://tex.stackexchange.com/questions/218378/forcing-subfigures-to-have-same-height-and-take-overall-x-of-linewidth-in-latex
\sbox\foursubbox{%
  \resizebox{\textwidth}{!}{%
    \includegraphics[height=3cm]{L1L2fig/sDice11}%
    \includegraphics[height=3cm]{L1L2fig/sDice11L2}%
    \includegraphics[height=3cm]{L1L2fig/sDice10}%
    \includegraphics[height=3cm]{L1L2fig/sDice10L2}%
  }%
}%
\setlength{\foursubht}{\ht\foursubbox}%

  \centering%
\subcaptionbox{$y=[1, 1]$; $L^1$ soft Dice\label{fig:sdice11L1}}{%
  \includegraphics[height=\foursubht]{L1L2fig/sDice11}%
}%
\subcaptionbox{$y=[1, 1]$; $L^2$ soft Dice\label{fig:sdice11L2}}{%
  \includegraphics[height=\foursubht]{L1L2fig/sDice11L2}%
}%
\subcaptionbox{$y=[1, 0]$; $L^1$ soft Dice\label{fig:sdice10L1}}{%
  \includegraphics[height=\foursubht]{L1L2fig/sDice10}%
}%
\subcaptionbox{$y=[1, 0]$; $L^2$ soft Dice\label{fig:sdice10L2}}{%
  \includegraphics[height=\foursubht]{L1L2fig/sDice10L2}%
}%
%   \begin{subfigure}[b]{0.25\textwidth}%
%      \centering%
%      \includegraphics[width=\linewidth]{histfig/BRATS_2018_decomp_new_model}%
%      \caption{BRATS 2018}% 
%   \end{subfigure}%
%   \begin{subfigure}[b]{0.25\textwidth}%
%      \centering%
%      \includegraphics[width=\linewidth]{histfig/POLYPS_decomp}%
%      \caption{PO18}%
%   \end{subfigure}%
%   \begin{subfigure}[b]{0.25\textwidth}%
%      \centering%
%      \includegraphics[width=\linewidth]{histfig/38_decomp_new_model}%
%      \caption{MO17}%
%   \end{subfigure}%
%   \begin{subfigure}[b]{0.25\textwidth}%
%      \centering%
%      \includegraphics[width=\linewidth]{histfig/ISLES_2018_decomp}%
%      \caption{ISLES 2018}%
%   \end{subfigure}%
  \caption{\review{Comparison between $L^1$ and $L^2$--based variants of the soft Dice loss for a two-pixel prediction $\tilde{y}=[\tilde{y}_0, \tilde{y}_1]$, and two different ground truth labels $y$. 
  The red dots indicate the values of the discrete Dice loss. 
  We see that the $L^2$ variants are flatter around the global minimum corresponding to the ground truth configuration.\label{fig:l1l2surfaces}}}%
\end{figure*}

==> TMI - Dice/appendices.tex <==
%\clearpage
% make supplementary counters different from main document
% \counterwithin{algorithm}{section}
% \counterwithin{definition}{section}
% \counterwithin{theorem}{section}
% \counterwithin{proposition}{section}
% \appendix

%\counterwithin{figure}{section}
%\counterwithin{table}{section}
%\counterwithin{equation}{section}


%\textbf{{\Large Supplementary material}} \\
%\pagenumbering{Roman}  % roman page numbers on supplementary

\section{MICCAI 2018 proceedings}\label{sec:MICCAI2018methodology}

In the introduction, it is stated that only 30\% of all MICCAI 2018 proceedings actually use a metric-sensitive loss function. This, even though the Dice score is reported as their evaluation metric. We categorized all MICCAI 2018 proceedings \cite{frangi2018medical} as indicated by the flowchart in Figure~\ref{fig:flowchart_proceedings_count}. From the total number of MICCAI 2018 proceedings (n = 372), there are 103 papers dealing with learning-based segmentation. Almost all of them (n=96) use the Dice score or Jaccard index to evaluate the performance of their algorithm, but only 28 proceedings report to use soft Dice or any of the other metric-sensitive loss functions described in this work. Many methods use cross-entropy or its weighted variant (n=38) and the rest have used a variety of other losses such as adverserial loss, focal loss, mean-squared-error, etc.

\begin{figure}[htb]
    \centering
    \def\svgwidth{\columnwidth}
    \input{flowchart/miccai_count.pdf_tex}
    \caption{Flowchart used for categorization of MICCAI 2018 proceedings. All segmentation papers are selected and from these, we retain all the papers that used DICE score for evaluation. We then analysed which type of loss function was used.}  \label{fig:flowchart_proceedings_count}
\end{figure}

==> TMI - Dice/boxplots/table_L1vsL2.tex <==
\begin{figure}[!htbp]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYYY}

        & BR18 &   IS17 &  IS18 & MO18 & PO18 & WM17 & WM17\textsuperscript{DM}  \\
        
        \rotatebox{90}{\hspace{5pt} DICE} &
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_BR18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_IS17_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_IS18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_MO18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_PO18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_WM17_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_WM17_DM_DICE.png}  \\ 
        
        \rotatebox{90}{\hspace{5pt} JACC} &
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_BR18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_IS17_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_IS18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_MO18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_PO18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_WM17_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/L1vsL2/L1vsL2_WM17_DM_JACCARD.png}  \\ 

    \end{tabularx}
    }
        \caption{\reviewminorpar Boxplots for the Dice scores and Jaccard indexes obtained for each dataset, using the $L^1$ and $L^2$ generalization for soft Dice loss.}
    \label{fig:boxplots_L1vsL2}
\end{figure}

==> TMI - Dice/boxplots/table_alternative_tversky.tex <==
\begin{figure*}[!htbp]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYYY}

        & BR18 &   IS17 &  IS18 & MO18 & PO18 & WM17 & WM17\textsuperscript{DM}  \\
        
        \rotatebox{90}{\hspace{20pt} F0.5} &
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_BR18_F0_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_IS17_F0_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_IS18_F0_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_MO18_F0_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_PO18_F0_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_WM17_F0_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_WM17_DM_F0_5_png.png}  \\ 
        
        \rotatebox{90}{\hspace{20pt} F1.0} &
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_BR18_F1_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_IS17_F1_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_IS18_F1_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_MO18_F1_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_PO18_F1_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_WM17_F1_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_WM17_DM_F1_0_png.png}  \\ 
    
        \rotatebox{90}{\hspace{20pt} F1.5} &
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_BR18_F1_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_IS17_F1_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_IS18_F1_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_MO18_F1_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_PO18_F1_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_WM17_F1_5_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_WM17_DM_F1_5_png.png}  \\ 

        \rotatebox{90}{\hspace{20pt} F2.0} &
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_BR18_F2_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_IS17_F2_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_IS18_F2_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_MO18_F2_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_PO18_F2_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_WM17_F2_0_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/alternative_tversky/alternative_tversky_WM17_DM_F2_0_png.png}  \\ 

    \end{tabularx}
    }
        \caption{\reviewminorpar Boxplots of the alternative F measures obtained for each dataset using the range of sTversky losses with varying alpha/beta.}
    \label{fig:boxplots_alternative_tversky}
\end{figure*}


==> TMI - Dice/boxplots/table_cropped.tex <==
\begin{figure}[!htbp]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYY}

        & 0.05 &   0.1 &  0.2 & 0.3 & 0.4 & 0.5   \\
        
        \rotatebox{90}{\hspace{5pt} DICE} &
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped005_PO18_DICE_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped010_PO18_DICE_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped020_PO18_DICE_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped030_PO18_DICE_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped040_PO18_DICE_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped050_PO18_DICE_png.png}  \\ 
        
        \rotatebox{90}{\hspace{5pt} JACC} &
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped005_PO18_JACCARD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped010_PO18_JACCARD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped020_PO18_JACCARD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped030_PO18_JACCARD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped040_PO18_JACCARD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/cropped/cropped050_PO18_JACCARD_png.png}  \\ 

    \end{tabularx}
    }
        \caption{\reviewminorpar Boxplots for the Dice scores and Jaccard indexes obtained for each virtual PO18 dataset and for networks trained with CE or sDice.}
    \label{fig:boxplots_cropped}
\end{figure}

==> TMI - Dice/boxplots/table_main.tex <==
\begin{figure*}[!htbp]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYYY}

        & BR18 &   IS17 &  IS18 & MO18 & PO18 & WM17 & WM17\textsuperscript{DM}  \\
        
        \rotatebox{90}{\hspace{20pt} DICE} &
        \includegraphics[width=\linewidth]{boxplots/main/main_BR18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_IS17_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_IS18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_MO18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_PO18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_WM17_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_WM17_DM_DICE.png}  \\ 
        
        \rotatebox{90}{\hspace{20pt} JACC} &
        \includegraphics[width=\linewidth]{boxplots/main/main_BR18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_IS17_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_IS18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_MO18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_PO18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_WM17_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main/main_WM17_DM_JACCARD.png}  \\ 

    \end{tabularx}
    }
        \caption{\reviewminorpar Boxplots for the Dice scores and Jaccard indexes obtained for each dataset, using a cross-entropy loss (CE, wCE) or a metric-sensitive loss (sDice, sJaccard, Lov\'{a}sz).}
    \label{fig:boxplots_main}
\end{figure*}


==> TMI - Dice/boxplots/table_main_tversky.tex <==
\begin{figure*}[!htbp]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYYY}

        & BR18 &   IS17 &  IS18 & MO18 & PO18 & WM17 & WM17\textsuperscript{DM}  \\
        
        \rotatebox{90}{\hspace{20pt} DICE} &
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_BR18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_IS17_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_IS18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_MO18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_PO18_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_WM17_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_WM17_DM_DICE.png}  \\ 
        
        \rotatebox{90}{\hspace{20pt} JACC} &
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_BR18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_IS17_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_IS18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_MO18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_PO18_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_WM17_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/main_tversky/main_tversky_WM17_DM_JACCARD.png}  \\ 

    \end{tabularx}
    }
        \caption{\reviewminorpar Boxplots for the Dice scores and Jaccard indexes obtained for all datasets using the range of sTversky losses with varying alpha/beta.}
    \label{fig:boxplots_main_tversky}
\end{figure*}


==> TMI - Dice/boxplots/table_multiclass.tex <==
\begin{figure}[!htbp]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYY}

        & All &   WT &  TC & ET  \\
        
        \rotatebox{90}{\hspace{5pt} DICE} &
        \includegraphics[width=\linewidth]{boxplots/multiclass/multiclass_All_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass/multiclass_WT_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass/multiclass_TC_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass/multiclass_ET_DICE.png}   \\ 
        
        \rotatebox{90}{\hspace{5pt} JACC} &
        \includegraphics[width=\linewidth]{boxplots/multiclass/multiclass_All_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass/multiclass_WT_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass/multiclass_TC_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass/multiclass_ET_JACCARD.png} \\ 

    \end{tabularx}
    }
        \caption{\reviewminorpar Boxplots for the Dice scores and Jaccard indexes obtained for the multi-class BRATS dataset using the original loss functions. Results are presented for the three volumes that were considered for evaluation during the challenge: whole tumor (WT), tumor core (TC) and enhancing tumor (ET). We also report the average across the three types (all).}
    \label{fig:boxplots_multiclass}
\end{figure}

==> TMI - Dice/boxplots/table_multiclass_tversky.tex <==
\begin{figure}[!htbp]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYY}

        & All &   WT &  TC & ET  \\
        
        \rotatebox{90}{\hspace{5pt} DICE} &
        \includegraphics[width=\linewidth]{boxplots/multiclass_tversky/multiclass_tversky_All_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass_tversky/multiclass_tversky_WT_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass_tversky/multiclass_tversky_TC_DICE.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass_tversky/multiclass_tversky_ET_DICE.png}   \\ 
        
        \rotatebox{90}{\hspace{5pt} JACC} &
        \includegraphics[width=\linewidth]{boxplots/multiclass_tversky/multiclass_tversky_All_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass_tversky/multiclass_tversky_WT_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass_tversky/multiclass_tversky_TC_JACCARD.png} &  
        \includegraphics[width=\linewidth]{boxplots/multiclass_tversky/multiclass_tversky_ET_JACCARD.png} \\ 

    \end{tabularx}
    }
        \caption{\reviewminorpar Boxplots for the Dice scores and Jaccard indexes obtained for the multi-class BRATS dataset using the range of sTversky
        losses with varying alpha/beta. Results are presented for the three volumes that were considered for evaluation during the challenge: whole tumor (WT), tumor core (TC) and enhancing tumor (ET). We also report the average across the three types (all).}
    \label{fig:boxplots_multiclass_tversky}
\end{figure}

==> TMI - Dice/boxplots/table_othermetrics.tex <==
\begin{figure}[!htbp]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYYY}

        & BR18 &   IS17 &  IS18 & MO18 & PO18 & WM17 & WM17\textsuperscript{DM}  \\
        
        \rotatebox{90}{\hspace{5pt} ACC} &
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_BR18_ACC_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_IS17_ACC_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_IS18_ACC_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_MO18_ACC_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_PO18_ACC_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_WM17_ACC_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_WM17_DM_ACC_png.png}  \\ 
        
        \rotatebox{90}{\hspace{5pt} HAU} &
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_BR18_HAU_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_IS17_HAU_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_IS18_HAU_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_MO18_HAU_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_PO18_HAU_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_WM17_HAU_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_WM17_DM_HAU_png.png}  \\ 
        
        \rotatebox{90}{\hspace{5pt} AVD} &
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_BR18_AVD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_IS17_AVD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_IS18_AVD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_MO18_AVD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_PO18_AVD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_WM17_AVD_png.png} &  
        \includegraphics[width=\linewidth]{boxplots/othermetrics/othermetrics_WM17_DM_AVD_png.png}  \\ 

    \end{tabularx}
    }
        \caption{\reviewminorpar Boxplots for the accuracy, Hausdorff distance and absolute volume difference obtained for each dataset, using a cross-entropy loss (CE, wCE) or a metric-sensitive loss (sDice, sAVD, Lov\'{a}sz).}
    \label{fig:boxplots_othermetrics}
\end{figure}

==> TMI - Dice/cropfig/crop_results_tbl.tex <==
\begin{tabularx}{\linewidth}{llXYYYYYY}
    \toprule
         & Loss & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{Dataset} $\rightarrow$}} & \reviewminor{0.05} & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\
    \midrule
\parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Dice}}}
      & CE    & & \reviewminor{\textit{0.627}} & \textit{0.645} &  \textit{0.673} &  \textit{0.691} &  \textit{0.730} &  \textit{0.757} \\
      & sDice & & \cellcolor{gray!50} \reviewminor{0.639} & \cellcolor{gray!50} 0.662 & \cellcolor{gray!50} 0.683 & \cellcolor{gray!50} 0.701 & \cellcolor{gray!50} 0.740 & \cellcolor{gray!50} 0.765 \\
    \midrule
    \parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Jacc.}}}
      & CE    & & \reviewminor{\textit{0.534}} & \textit{0.552} &  \textit{0.579} &  \textit{0.597} &  \textit{0.639} &  \textit{0.672} \\
      & sDice & & \cellcolor{gray!50} \reviewminor{0.541} & \cellcolor{gray!50} 0.564 & \cellcolor{gray!50} 0.584 & \cellcolor{gray!50} 0.604 & \cellcolor{gray!50} 0.646 & \cellcolor{gray!50} 0.676 \\
         
    \bottomrule
\end{tabularx}

==> TMI - Dice/cropfig/cropfig.tex <==
\begin{figure}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
        \includegraphics{cropfig/p001_01_N_WLImp4-00001_005.png} & \includegraphics{cropfig/p001_01_N_WLImp4-00001_010.png} & \includegraphics{cropfig/p001_01_N_WLImp4-00001_020.png} \\
        \includegraphics{cropfig/p001_01_N_WLImp4-00001_030.png} & \includegraphics{cropfig/p001_01_N_WLImp4-00001_040.png} & \includegraphics{cropfig/p001_01_N_WLImp4-00001_050.png}
    \end{tabular}
    }
    \caption{\reviewminor{For each foreground to background ratio in red, a rectangular mask is created with the same aspect ratio as the original image and which contains the entire polyp (or part of it if not possible) in green.}}
    \label{fig:cropfig}
\end{figure}

==> TMI - Dice/empirical_results_tbl.tex <==
%% Results for old model:
% \begin{tabularx}{\linewidth}{lsXYYYYY}
%     \toprule
%     & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice score}}} 
%     & BR18 & & 0.768 & 0.735 & 0.823 & 0.823 & 0.827 \\
%     & IS17 & & 0.260 & 0.311 & 0.331 & 0.321 & 0.305 \\
%     & IS18 & & 0.463 & 0.474 & 0.538 & 0.528 & 0.508 \\
%     & MO17 & & 0.930 & 0.860 & 0.932 & 0.931 & 0.932 \\
%     & PO18 & & 0.635 & 0.602 & 0.656 & 0.651 & 0.649 \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard index}}}
%     & BR18 & & 0.654 & 0.602 & 0.717 & 0.720 & 0.722 \\
%     & IS17 & & 0.177 & 0.212 & 0.227 & 0.217 & 0.204 \\
%     & IS18 & & 0.345 & 0.344 & 0.407 & 0.399 & 0.382 \\
%     & MO17 & & 0.873 & 0.769 & 0.877 & 0.875 & 0.877 \\
%     & PO18 & & 0.541 & 0.488 & 0.559 & 0.554 & 0.553 \\
%     \bottomrule
% \end{tabularx}
% \begin{tabularx}{\linewidth}{lsXYYYYY}
%     \toprule
%     & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice score}}} 
%     & BR18 & & \textit{0.768} & \underline{\textit{0.735}} & 0.823 & 0.823 & \textbf{0.827} \\
%     & IS17 & & \underline{\textit{0.260}} & 0.311 & 0.331 & 0.321 & 0.305 \\
%     & IS18 & & \textit{0.463} & \textit{0.474} & \textbf{0.538} & 0.528 & \underline{0.508} \\
%     & MO17 & & 0.930 & \underline{\textit{0.860}} & 0.932 & 0.931 & 0.932 \\
%     & PO18 & & \textit{0.635} & \underline{\textit{0.602}} & 0.656 & 0.651 & 0.649 \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard index}}}
%     & BR18 & & \textit{0.654} & \underline{\textit{0.602}} & 0.717 & 0.720 & 0.722 \\
%     & IS17 &  & \underline{\textit{0.177}} & 0.212 & 0.227 & 0.217 & 0.204 \\
%     & IS18 &  & \textit{0.345} & \textit{0.344} & \textbf{0.407} & 0.399 & \underline{0.382} \\
%     & MO17 & & 0.873 & \underline{\textit{0.769}} & 0.877 & 0.875 & 0.877 \\
%     & PO18 & & \textit{0.541} & \underline{\textit{0.488}} & 0.559 & 0.554 & 0.553 \\
%     \bottomrule
% \end{tabularx}

%% Results for new model:
% \begin{tabularx}{\linewidth}{lsXYYYYY}
%     \toprule
%     & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice score}}} 
%     & BR18 & & 0.848 & 0.805 & 0.870 & 0.868 & 0.871 \\
%     & IS17 & & 0.281 & 0.293 & 0.362 & 0.362 & 0.357 \\
%     & IS18 & & 0.399 & 0.425 & 0.526 & 0.528 & 0.386 \\
%     & MO17 & & 0.942 & 0.903 & 0.944 & 0.942 & 0.944 \\
%     & PO18 & & 0.635 & 0.602 & 0.656 & 0.651 & 0.649 \\ %old model == new model
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard index}}}
%     & BR18 & & 0.751 & 0.693 & 0.780 & 0.780 & 0.784 \\
%     & IS17 & & 0.191 & 0.199 & 0.244 & 0.246 & 0.245 \\
%     & IS18 & & 0.295 & 0.304 & 0.396 & 0.400 & 0.281 \\
%     & MO17 & & 0.894 & 0.835 & 0.897 & 0.896 & 0.896 \\
%     & PO18 & & 0.541 & 0.488 & 0.559 & 0.554 & 0.553 \\ %old model == new model
%     \bottomrule
% \end{tabularx}
\begin{tabularx}{\linewidth}{lsXYY|YYY}
    \toprule
    & & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{group} $\rightarrow$}} & \multicolumn{2}{c}{CE-based} & \multicolumn{3}{c}{Metric-sensitive} \\
    \midrule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    & BR18 & & 0.848 & \textit{0.808} & \cellcolor{gray!50} 0.870 & \cellcolor{gray!50}0.868 & \cellcolor{gray!50}0.871 \\
    & IS17 & & 0.281 & 0.310 & \cellcolor{gray!50} 0.362 & \cellcolor{gray!50} 0.363 & \cellcolor{gray!50} 0.357 \\
    & IS18 & & 0.463 & 0.487 & \cellcolor{gray!50} 0.538 & 0.528 & 0.508 \\
    & MO18 & & \cellcolor{gray!50} 0.942 & \textit{0.903} & \cellcolor{gray!50} 0.944 & \cellcolor{gray!50} 0.942 & \cellcolor{gray!50} 0.944 \\
    & PO18 & & 0.635 & \textit{0.602} & \cellcolor{gray!50} 0.656 & \cellcolor{gray!50} 0.651 & \cellcolor{gray!50} 0.649 \\
    & \review{WM17} & & \review{0.672} & \review{\textit{0.492}} & \cellcolor{gray!50} \review{0.712} & \cellcolor{gray!50} \review{0.712} & \review{0.700} \\
    & \review{WM17\textsuperscript{DM}} & & \review{0.671} & \review{\textit{0.383}} & \cellcolor{gray!50} \review{0.717} & \cellcolor{gray!50} \review{0.714} & \cellcolor{gray!50} \review{0.711} \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    & BR18 & & 0.751 & \textit{0.695} & \cellcolor{gray!50} 0.780 & \cellcolor{gray!50} 0.780 & \cellcolor{gray!50} 0.784 \\
    & IS17 & & 0.191 & 0.212 & \cellcolor{gray!50} 0.244 & \cellcolor{gray!50} 0.246 & \cellcolor{gray!50} 0.245 \\
    & IS18 & & 0.345 & 0.357 & \cellcolor{gray!50} 0.407 & 0.399 & 0.382 \\
    & MO18 & & \cellcolor{gray!50} 0.894 & \textit{0.835} & \cellcolor{gray!50} 0.897 & \cellcolor{gray!50}  0.896 & \cellcolor{gray!50} 0.896 \\
    & PO18 & & 0.541 & \textit{0.488} & \cellcolor{gray!50} 0.559 & \cellcolor{gray!50} 0.554 & \cellcolor{gray!50} 0.553 \\
    & \review{WM17} & & \review{0.530} & \review{\textit{0.355}} & \cellcolor{gray!50} \review{0.571} & \cellcolor{gray!50} \review{0.573} & \review{0.558} \\
    & \review{WM17\textsuperscript{DM}} & & \review{0.529} & \review{\textit{0.273}} & \cellcolor{gray!50} \review{0.577} & \cellcolor{gray!50} \review{0.576} & \cellcolor{gray!50} \review{0.572} \\
    \bottomrule
\end{tabularx}


==> TMI - Dice/histfig/histfig.tex <==
\begin{figure*}[htbp]%
% https://tex.stackexchange.com/questions/218378/forcing-subfigures-to-have-same-height-and-take-overall-x-of-linewidth-in-latex
% preliminary
\sbox\foursubbox{%
  \resizebox{\textwidth}{!}{%
    \includegraphics[height=3cm]{histfig/BRATS_2018_decomp_new_model}%
    \includegraphics[height=3cm]{histfig/ISLES_2018_decomp}%
    \includegraphics[height=3cm]{histfig/38_decomp_new_model}%
    \includegraphics[height=3cm]{histfig/POLYPS_decomp}%
  }%
}%
\setlength{\foursubht}{\ht\foursubbox}%
%
  \centering%
\subcaptionbox{BR18\label{fig:areaBR}}{%
  \includegraphics[height=\foursubht]{histfig/BRATS_2018_decomp_new_model}%
}%
\subcaptionbox{IS18\label{fig:areaIS}}{%
  \includegraphics[height=\foursubht]{histfig/ISLES_2018_decomp}%
}%
\subcaptionbox{MO17\label{fig:areaMO}}{%
  \includegraphics[height=\foursubht]{histfig/38_decomp_new_model}%
}%
\subcaptionbox{PO18\label{fig:areaPO}}{%
  \includegraphics[height=\foursubht]{histfig/POLYPS_decomp}%
}%
%   \begin{subfigure}[b]{0.25\textwidth}%
%      \centering%
%      \includegraphics[width=\linewidth]{histfig/BRATS_2018_decomp_new_model}%
%      \caption{BRATS 2018}% 
%   \end{subfigure}%
%   \begin{subfigure}[b]{0.25\textwidth}%
%      \centering%
%      \includegraphics[width=\linewidth]{histfig/POLYPS_decomp}%
%      \caption{PO18}%
%   \end{subfigure}%
%   \begin{subfigure}[b]{0.25\textwidth}%
%      \centering%
%      \includegraphics[width=\linewidth]{histfig/38_decomp_new_model}%
%      \caption{MO17}%
%   \end{subfigure}%
%   \begin{subfigure}[b]{0.25\textwidth}%
%      \centering%
%      \includegraphics[width=\linewidth]{histfig/ISLES_2018_decomp}%
%      \caption{ISLES 2018}%
%   \end{subfigure}%
  \caption{Dice score as a function of object size (\# foreground pixels in \%) for BR18 (a), IS18 (b), MO17 (c) and PO18 (d). The results for IS17 \review{and WM17} are omitted due to the small dataset size and lack of statistical relevance. 
  For visualization purposes, the Dice scores are averaged within every 10th percentile (bordered by the dashed lines). 
  The superior performance for metric-sensitive losses holds across the entire range of object sizes.\label{fig:dice_size}}%
\end{figure*}

==> TMI - Dice/l1vsl2_tbl.tex <==
\begin{tabularx}{\linewidth}{llXYYYYYYY}
    \toprule
         & Loss & \multicolumn{1}{l}{\lapbox[0.5\width]{0.5em}{\emph{Data} $\rightarrow$}} & BR18 & IS17 & IS18 & MO17 & PO18 & \review{WM17} & \review{WM17\textsuperscript{DM}} \\
    \midrule
    \parbox[t]{1mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Dice}}}
      & $L^1$   & &  0.870 &  0.362 &  \cellcolor{gray!50} 0.538 &  0.944 &  \cellcolor{gray!50} 0.656 & \review{0.712} & \cellcolor{gray!50} \review{0.717} \\
      & $L^2$   & &  0.869 &  0.358 &  \textit{0.525} &  0.943 &  \textit{0.639} & \review{0.708} & \review{\textit{0.703}}\\
    \midrule
    \parbox[t]{1mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Jacc.}}}
      & $L^1$   & &  0.780 &  0.244 & \cellcolor{gray!50} 0.407 &  0.897 &  \cellcolor{gray!50} 0.598 & \review{0.571} & \cellcolor{gray!50} \review{0.577} \\
      & $L^2$   & &  0.780 &  0.245 & \textit{0.395} &  0.896 &  \textit{0.567} & \review{0.566} & \review{\textit{0.563}} \\
         
    \bottomrule
\end{tabularx}

==> TMI - Dice/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> TMI - Dice/losses_qual/losses_qual.tex <==
\begin{sidewaysfigure*}[p!]
    \centering

    \begin{tabularx}{0.75\textheight}{cYYYYYYY}
        & Original & Ground truth & CE & wCE & sDice & sJaccard & Lov\'{a}sz
    \end{tabularx}

    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{0.75\textheight}{l @{\hspace{2pt}} XXXXXXX}
    
        \rotatebox{90}{\hspace{20pt} BR18} &
        \includegraphics[width=\linewidth]{losses_qual/BR18/new_model/input_ce-ce_median_overlay.png} & 
        \includegraphics[width=\linewidth]{losses_qual/BR18/new_model/gt_ce-ce_median.png} & 
        \includegraphics[width=\linewidth]{losses_qual/BR18/new_model/CE-CE.png} &
        \includegraphics[width=\linewidth]{losses_qual/BR18/new_model/CE-wCE.png} &
        \includegraphics[width=\linewidth]{losses_qual/BR18/new_model/CE-DICE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/BR18/new_model/CE-JACCARD.png} &
        \includegraphics[width=\linewidth]{losses_qual/BR18/new_model/CE-LOVASZ.png} \\
       
        \rotatebox{90}{\hspace{25pt} IS17} &
        \includegraphics[width=\linewidth]{losses_qual/IS17/new_model/input_ce-ce_median_overlay.png} & 
        \includegraphics[width=\linewidth]{losses_qual/IS17/new_model/gt_ce-ce_median.png} &
        \includegraphics[width=\linewidth]{losses_qual/IS17/new_model/CE-CE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/IS17/new_model/CE-wCE.png} &
        \includegraphics[width=\linewidth]{losses_qual/IS17/new_model/CE-DICE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/IS17/new_model/CE-JACCARD.png} &
        \includegraphics[width=\linewidth]{losses_qual/IS17/new_model/CE-LOVASZ.png} \\
  
        \rotatebox{90}{\hspace{25pt} IS18} &
        \includegraphics[width=\linewidth]{losses_qual/IS18/old_model/input_ce-ce_median_overlay.png} & 
        \includegraphics[width=\linewidth]{losses_qual/IS18/old_model/gt_ce-ce_median.png} &
        \includegraphics[width=\linewidth]{losses_qual/IS18/old_model/CE-CE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/IS18/old_model/CE-wCE.png} &
        \includegraphics[width=\linewidth]{losses_qual/IS18/old_model/CE-DICE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/IS18/old_model/CE-JACCARD.png} &
        \includegraphics[width=\linewidth]{losses_qual/IS18/old_model/CE-LOVASZ.png} \\ 
        
        \rotatebox{90}{\hspace{20pt} MO17} &
        \includegraphics[width=\linewidth]{losses_qual/MO17/new_model/input_ce-ce_median_overlay.png} & 
        \includegraphics[width=\linewidth]{losses_qual/MO17/new_model/gt_ce-ce_median.png} &
        \includegraphics[width=\linewidth]{losses_qual/MO17/new_model/CE-CE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/MO17/new_model/CE-wCE.png} &
        \includegraphics[width=\linewidth]{losses_qual/MO17/new_model/CE-DICE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/MO17/new_model/CE-JACCARD.png} &
        \includegraphics[width=\linewidth]{losses_qual/MO17/new_model/CE-LOVASZ.png} \\
        
        \rotatebox{90}{\hspace{5pt} PO18} &
        \includegraphics[width=\linewidth]{losses_qual/POLYPS/p014_03_R_BLImp4-00001_orig_result.png} &
        \includegraphics[width=\linewidth]{losses_qual/POLYPS/p014_03_R_BLImp4-00001_ann.png} &
        \includegraphics[width=\linewidth]{losses_qual/POLYPS/p014_03_R_BLImp4-00001_CE_result.png} & \includegraphics[width=\linewidth]{losses_qual/POLYPS/p014_03_R_BLImp4-00001_wCE_result.png} &
        \includegraphics[width=\linewidth]{losses_qual/POLYPS/p014_03_R_BLImp4-00001_dice_result.png} & \includegraphics[width=\linewidth]{losses_qual/POLYPS/p014_03_R_BLImp4-00001_jaccard_result.png} &
        \includegraphics[width=\linewidth]{losses_qual/POLYPS/p014_03_R_BLImp4-00001_lovasz_result.png} \\ 
        
        \rotatebox{90}{\hspace{45pt} \review{WM17}} &
        \includegraphics[width=\linewidth]{losses_qual/WM17/new_model/input_ce-ce_median_overlay.png} & 
        \includegraphics[width=\linewidth]{losses_qual/WM17/new_model/gt_ce-ce_median.png} &
        \includegraphics[width=\linewidth]{losses_qual/WM17/new_model/CE-CE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/WM17/new_model/CE-wCE.png} &
        \includegraphics[width=\linewidth]{losses_qual/WM17/new_model/CE-DICE.png} & 
        \includegraphics[width=\linewidth]{losses_qual/WM17/new_model/CE-JACCARD.png} &
        \includegraphics[width=\linewidth]{losses_qual/WM17/new_model/CE-LOVASZ.png} \\
    \end{tabularx}

    \caption{\review{A qualitative evaluation of the resulting predictions from networks trained with CE, wCE, sDice, sJaccard and Lov\'{a}sz, columns 3-7, respectively. The predicted delineations are obtained after thresholding at 0.5 and are overlayed in red. The original images inputted to the network (or part of) are shown on the left. The ground truths are shown in the second column and their delineations are overlayed in blue on the predictions. The slices shown had a median Dice, both across cases and within one case (having a minimum of one foreground pixel), for the CE model and were checked visually for being representative.}}
    \label{fig:losses_qual}
\end{sidewaysfigure*}

==> TMI - Dice/multiclass/multiclass_results.tex <==
% \begin{tabularx}{\linewidth}{lsXYYYY}
%     \toprule
%     & Loss & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{Type} $\rightarrow$}} & All & Whole & Core & Active \\
%     \midrule
%     \parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Dice}}}
%     & CE & & 0.638 & 0.798 & 0.620 & 0.498 \\
%     & sDice & & \textbf{0.740} & \textbf{0.849} & \textbf{0.725} & \textbf{0.646} \\
%     \midrule
%     \parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Jacc}}}
%     & CE & & 0.522 & 0.683 & 0.487 & 0.395 \\
%     & sDice & & \textbf{0.632} & \textbf{0.753} & \textbf{0.609} & \textbf{0.534} \\
%     \bottomrule
% \end{tabularx}

% Results for new model:
% \begin{tabularx}{\linewidth}{lsXYYYYY}
%     \toprule
%     & Type & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice score}}} 
%     & All    & & 0.639 & 0.665 & 0.740 & 0.746 & 0.716 \\
%     & Whole  & & 0.798 & 0.799 & 0.849 & 0.857 & 0.858 \\
%     & Core   & & 0.620 & 0.635 & 0.725 & 0.737 & 0.692 \\
%     & Active & & 0.498 & 0.560 & 0.646 & 0.645 & 0.598 \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard index}}}
%     & All    & & 0.522 & 0.554 & 0.632 & 0.642 & 0.606 \\
%     & Whole  & & 0.683 & 0.688 & 0.753 & 0.765 & 0.766 \\
%     & Core   & & 0.487 & 0.518 & 0.609 & 0.627 & 0.569 \\
%     & Active & & 0.395 & 0.456 & 0.534 & 0.534 & 0.484 \\
%     \bottomrule
% \end{tabularx}
\begin{tabularx}{\linewidth}{llXYY|YYY}
    \toprule
    & & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{group} $\rightarrow$}} & \multicolumn{2}{c}{CE-based} & \multicolumn{3}{c}{Metric-sensitive} \\
    \midrule
    & Type & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    & All   & & 0.639 & 0.665 & 0.740 & \cellcolor{gray!50} 0.747 & 0.716 \\
    & WT    & & 0.798 & 0.799 & 0.849 & \cellcolor{gray!50}0.859 & \cellcolor{gray!50}0.858 \\
    & TC    & & 0.620 & 0.636 & 0.725 & \cellcolor{gray!50}0.737 & 0.692 \\
    & ET    & & 0.498 & 0.560 & \cellcolor{gray!50}0.646 & \cellcolor{gray!50}0.645 & 0.598 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    & All & & 0.522 & 0.554 & 0.632 & \cellcolor{gray!50}0.643 & 0.606 \\
    & WT  & & 0.683 & 0.688 & 0.753 & \cellcolor{gray!50}0.767 & \cellcolor{gray!50}0.766 \\
    & TC  & & 0.487 & 0.518 & 0.609 & \cellcolor{gray!50}0.627 & 0.569 \\
    & ET  & & 0.395 & 0.456 & \cellcolor{gray!50}0.534 & \cellcolor{gray!50}0.534 & 0.484 \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/multiclass/multiclass_tversky_results.tex <==
% Results for new model:
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Type & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & \review{0.75/0.75} & \review{1.0/1.0} \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    &All &        &        0.649 &        0.702 &        0.725 &        0.739 & 0.740 &        0.738 &        0.709 &        0.704 &        0.649 &   \cellcolor{gray!50}     \review{0.741} & \cellcolor{gray!50}\review{0.747} \\
    &WT &        &        0.771 &        0.822 &        0.844 &        0.853 & 0.849 &        0.848 &        0.826 &        0.816 &        0.757 &   \cellcolor{gray!50}     \review{0.858} & \cellcolor{gray!50}\review{0.859} \\
    &TC &        &        0.652 &        0.703 &        0.724 &     \cellcolor{gray!50}   0.735 & 0.725 &        0.725 &        0.687 &        0.686 &        0.623 &        \cellcolor{gray!50}\review{0.731} & \cellcolor{gray!50}\review{0.737} \\
    &ET &        &        \textit{0.525} &        0.582 &        0.606 &        0.631 & \cellcolor{gray!50}0.646 &   \cellcolor{gray!50}     0.642 &        0.614 &        0.611 &        0.568 &     \cellcolor{gray!50}   \review{0.634} &\cellcolor{gray!50} \review{0.645} \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    &All &        &        0.517 &        0.580 &        0.610 &        0.630 & 0.632 &        0.629 &        0.595 &        0.586 &        0.521 &        \review{0.634} & \cellcolor{gray!50}\review{0.643} \\
    &WT &        &        0.640 &        0.711 &        0.742 &        0.757 & 0.753 &        0.750 &        0.719 &        0.704 &        0.627 &       \cellcolor{gray!50} \review{0.765} & \cellcolor{gray!50}\review{0.767} \\
    &TC &        &        0.513 &        0.572 &        0.602 &        0.617 & 0.609 &        0.609 &        0.567 &        0.563 &        0.493 &        \review{0.615} &\cellcolor{gray!50} \review{0.627} \\
    &ET &        &        0.397 &        0.457 &        0.487 &        0.515 & \cellcolor{gray!50}0.534 &  \cellcolor{gray!50}      0.528 &        0.500 &        0.491 &        0.444 &        \review{0.522} &\cellcolor{gray!50} \review{0.534} \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/other_metrics/tbl.tex <==
\begin{tabularx}{\linewidth}{llXYYYYY}
    \toprule
         & Loss & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{Dataset} $\rightarrow$}} & BR18 & IS17 & IS18 & WM17 & WM17\textsuperscript{DM} \\
    \midrule
    \parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{ACC}}}
      & CE    & & \textit{0.997} & \cellcolor{gray!50} 0.995 & \cellcolor{gray!50} 0.989 & 0.999 & 0.999 \\
      & sDice & & \cellcolor{gray!50} 0.998 & \textit{0.993} & \textit{0.988} & 0.999 & 0.999 \\
    \midrule
    \parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{HDD}}}
      & CE    & & 22.673 & \textit{73.102} & \textit{42.994} & 34.210 & 30.526 \\
      & sDice & & 22.911 & \cellcolor{gray!50} 47.043 & \cellcolor{gray!50} 33.366 & 34.806 & 28.695 \\
    \midrule
    \parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{AVD}}}
      & CE    & & \textit{15.579} & 21.042 & 12.029 & \textit{5.628} & \textit{5.865} \\
      & sDice & & \cellcolor{gray!50} 13.375 & 35.895 & 11.954 & \cellcolor{gray!50} 3.895 & \cellcolor{gray!50} 4.064 \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/significances_tbl.tex <==
% \begin{tabularx}{\linewidth}{ll|Y|Y|Y|Y|Y}
% \toprule
%      & Loss &   CE &  wCE & DICE & JACC & LOVA \\
% Dataset & Loss &      &      &      &      &      \\
% \midrule
% MO18 & CE &  000 &  111 &  000 &  000 &  000 \\
%      & wCE &  000 &  000 &  000 &  000 &  000 \\
%      & DICE &  011 &  111 &  000 &  000 &  000 \\
%      & JACC &  000 &  111 &  000 &  000 &  000 \\
%      & LOVA &  011 &  111 &  000 &  000 &  000 \\
% BR18 & CE &  000 &  111 &  000 &  000 &  000 \\
%      & wCE &  000 &  000 &  000 &  000 &  000 \\
%      & DICE &  111 &  111 &  000 &  000 &  000 \\
%      & JACC &  111 &  111 &  100 &  000 &  000 \\
%      & LOVA &  111 &  111 &  111 &  010 &  000 \\
% IS17 & CE &  000 &  100 &  100 &  100 &  100 \\
%      & wCE &  011 &  000 &  000 &  000 &  000 \\
%      & DICE &  011 &  010 &  000 &  000 &  011 \\
%      & JACC &  011 &  100 &  100 &  000 &  000 \\
%      & LOVA &  011 &  000 &  000 &  000 &  000 \\
% IS18 & CE &  000 &  100 &  100 &  100 &  100 \\
%      & wCE &  000 &  000 &  000 &  000 &  000 \\
%      & DICE &  011 &  111 &  000 &  011 &  011 \\
%      & JACC &  011 &  111 &  000 &  000 &  011 \\
%      & LOVA &  011 &  111 &  000 &  000 &  000 \\
% PO18 & CE &  000 &  111 &  000 &  100 &  000 \\
%      & wCE &  000 &  000 &  000 &  000 &  000 \\
%      & DICE &  011 &  111 &  000 &  000 &  000 \\
%      & JACC &  011 &  111 &  000 &  000 &  000 \\
%      & LOVA &  011 &  111 &  000 &  000 &  000 \\
% \bottomrule
% \end{tabularx}

\begin{tabularx}{\linewidth}{ll|Y|Y|Y|Y|Y}
\toprule
     & Train loss: &   CE &  wCE & sDice & sJaccard & Lov\`{a}sz \\
Dataset: & Train loss: &      &      &      &      &      \\
\midrule
BR18 & CE &  00 &  11 &  00 &  00 &  00 \\
     & wCE &  00 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  11 &  00 &  00 &  00 \\
     & sJaccard &  11 &  11 &  00 &  00 &  00 \\
     & Lov\`{a}sz &  11 &  11 &  11 &  10 &  00 \\
IS17 & CE &  00 &  00 &  00 &  00 &  00 \\
     & wCE &  11 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  10 &  00 &  00 &  11 \\
     & sJaccard &  11 &  00 &  00 &  00 &  00 \\
     & Lov\`{a}sz &  11 &  00 &  00 &  00 &  00 \\
IS18 & CE &  00 &  00 &  00 &  00 &  00 \\
     & wCE &  00 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  11 &  00 &  11 &  11 \\
     & sJaccard &  11 &  11 &  00 &  00 &  11 \\
     & Lov\`{a}sz &  11 &  11 &  00 &  00 &  00 \\
MO17 & CE &  00 &  11 &  00 &  00 &  00 \\
     & wCE &  00 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  11 &  00 &  00 &  00 \\
     & sJaccard &  00 &  11 &  00 &  00 &  00 \\
     & Lov\`{a}sz &  11 &  11 &  00 &  00 &  00 \\
PO18 & CE &  00 &  11 &  00 &  00 &  00 \\
     & wCE &  00 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  11 &  00 &  00 &  00 \\
     & sJaccard &  11 &  11 &  00 &  00 &  00 \\
     & Lov\`{a}sz &  11 &  11 &  00 &  00 &  00 \\
\bottomrule
\end{tabularx}

==> TMI - Dice/supplementary_data/crop_results_stderr.tex <==
\begin{tabularx}{\linewidth}{llXYYYYY}
    \toprule
         & Loss & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{Dataset} $\rightarrow$}} & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\
    \midrule
\parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Dice}}}
      & CE    & &  0.010 &  0.009 &  0.009 &  0.009 &  0.008 \\
      & sDice & &  0.009 &  0.009 &  0.009 &  0.008 &  0.008 \\
    \midrule
    \parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Jacc.}}}
      & CE    & &  0.009 &  0.009 &  0.009 &  0.009 &  0.009 \\
      & sDice & &  0.009 &  0.009 &  0.009 &  0.008 &  0.008 \\
         
    \bottomrule
\end{tabularx}

==> TMI - Dice/supplementary_data/empirical_results_stderr.tex <==
% Std Error
\begin{tabularx}{\linewidth}{lsXYYYYY}
    \toprule
    & & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{group} $\rightarrow$}} & \multicolumn{2}{c}{CE-based} & \multicolumn{3}{c}{Metric-sensitive} \\
    \midrule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    & BR18 &        & 0.007 & 0.008 & 0.006 & 0.007 & 0.006 \\
    & IS17 &        & 0.039 & 0.039 & 0.034 & 0.035 & 0.038 \\
    & IS18 &        & 0.029 & 0.026 & 0.027 & 0.027 & 0.028 \\
    & MO18 &        & 0.003 & 0.005 & 0.003 & 0.003 & 0.002 \\
    & PO18 &        & 0.010 & 0.009 & 0.009 & 0.010 & 0.010 \\
    & WM17 &        & 0.023 & 0.029 & 0.019 & 0.020 & 0.020 \\
    & WM17\textsuperscript{DM} &        & 0.022 & 0.034 & 0.019 & 0.020 & 0.021 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    & BR18 &        & 0.009 & 0.009 & 0.008 & 0.008 & 0.008 \\
    & IS17 &        & 0.029 & 0.030 & 0.027 & 0.028 & 0.029 \\
    & IS18 &        & 0.025 & 0.023 & 0.023 & 0.024 & 0.024 \\
    & MO18 &        & 0.004 & 0.006 & 0.004 & 0.004 & 0.004 \\
    & PO18 &        & 0.009 & 0.008 & 0.009 & 0.009 & 0.009 \\
    & WM17 &        & 0.024 & 0.025 & 0.021 & 0.022 & 0.022 \\
    & WM17\textsuperscript{DM} &        & 0.024 & 0.029 & 0.021 & 0.022 & 0.023 \\
    \bottomrule
\end{tabularx}

% IQR
% \begin{tabularx}{\linewidth}{lsXYYYYY}
%     \toprule
%     & & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{group} $\rightarrow$}} & \multicolumn{2}{c}{CE-based} & \multicolumn{3}{c}{Metric-sensitive} \\
%     \midrule
%     & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice}}} 
%     &BR18 &        & 0.097 & 0.134 & 0.081 & 0.083 & 0.084 \\
%     &IS17 &        & 0.466 & 0.473 & 0.335 & 0.357 & 0.421 \\
%     &IS18 &        & 0.479 & 0.322 & 0.324 & 0.318 & 0.379 \\
%     &MO18 &        & 0.029 & 0.054 & 0.031 & 0.031 & 0.029 \\
%     &PO18 &        & 0.462 & 0.385 & 0.389 & 0.395 & 0.417 \\
%     &WM17 &        & 0.228 & 0.291 & 0.186 & 0.186 & 0.176 \\
%     &WM17\textsuperscript{DM} &        & 0.238 & 0.456 & 0.195 & 0.203 & 0.215 \\   
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
%     &BR18 &        & 0.152 & 0.197 & 0.130 & 0.135 & 0.137 \\
%     &IS17 &        & 0.304 & 0.344 & 0.251 & 0.270 & 0.309 \\
%     &IS18 &        & 0.422 & 0.295 & 0.317 & 0.310 & 0.356 \\
%     &MO18 &        & 0.053 & 0.093 & 0.056 & 0.057 & 0.053 \\
%     &PO18 &        & 0.537 & 0.426 & 0.472 & 0.477 & 0.500 \\
%     &WM17 &        & 0.269 & 0.259 & 0.229 & 0.231 & 0.215 \\
%     &WM17\textsuperscript{DM} &        & 0.280 & 0.354 & 0.243 & 0.252 & 0.264 \\
%     \bottomrule
% \end{tabularx}


==> TMI - Dice/supplementary_data/l1vsl2_stderr.tex <==
\begin{tabularx}{\linewidth}{llXYYYYYYY}
    \toprule
         & Loss & \multicolumn{1}{l}{\lapbox[0.5\width]{0.5em}{\emph{Data} $\rightarrow$}} & BR18 & IS17 & IS18 & MO17 & PO18 & WM17 & WM17\textsuperscript{DM} \\
    \midrule
    \parbox[t]{1mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Dice}}}
      & $L^1$   & &  0.006 &  0.034 &  0.027 &  0.003 &  0.009 & 0.019 & 0.019 \\
      & $L^2$   & &  0.006 &  0.037 &  0.027 &  0.002 &  0.011   & 0.019 & 0.020\\
    \midrule
    \parbox[t]{1mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Jacc.}}}
      & $L^1$   & &  0.008 &  0.027 &  0.023 &  0.004 &  0.009 & 0.021 & 0.021 \\
      & $L^2$   & &  0.008 &  0.029 &  0.024 &  0.004 &  0.011   & 0.021 & 0.023 \\
         
    \bottomrule
\end{tabularx}

==> TMI - Dice/supplementary_data/multiclass_results_stderr.tex <==
\begin{tabularx}{\linewidth}{llXYY|YYY}
    \toprule
    & & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{group} $\rightarrow$}} & \multicolumn{2}{c}{CE-based} & \multicolumn{3}{c}{Metric-sensitive} \\
    \midrule
    & Type & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    & All & & 0.011 & 0.012 & 0.010 & 0.010 & 0.010 \\
    & WT  & & 0.008 & 0.009 & 0.007 & 0.007 & 0.007 \\
    & TC  & & 0.014 & 0.016 & 0.013 & 0.014 & 0.014 \\
    & ET  & & 0.020 & 0.019 & 0.017 & 0.017 & 0.018 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    & All    & & 0.010 & 0.012 & 0.010 & 0.010 & 0.010 \\
    & WT     & & 0.010 & 0.010 & 0.009 & 0.008 & 0.008 \\
    & TC     & & 0.013 & 0.016 & 0.014 & 0.014 & 0.014 \\
    & ET     & & 0.018 & 0.018 & 0.016 & 0.016 & 0.016 \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/supplementary_data/multiclass_tversky_fmeasures.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY}
    \toprule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{BR18}}} 
    & F0.5 & & 0.739 & 0.806 & 0.841 & 0.853 & 0.878 & 0.890 & 0.896 & 0.894 & 0.879 \\
    & F1.0 & & 0.801 & 0.844 & 0.859 & 0.863 & 0.870 & 0.867 & 0.857 & 0.831 & 0.787 \\
    & F1.5 & & 0.850 & 0.874 & 0.875 & 0.873 & 0.867 & 0.855 & 0.837 & 0.798 & 0.741 \\ %old model
    & F2.0 & & 0.882 & 0.893 & 0.885 & 0.880 &  0.867 & 0.850 & 0.827 & 0.782 & 0.719 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS17}}} 
    & F0.5 & & 0.316 & 0.318 & 0.358 & 0.372 & 0.368 & 0.367 & 0.387 & 0.382 & 0.363 \\
    & F1.0 & & 0.352 & 0.345 & 0.374 & 0.374 & 0.362 & 0.346 & 0.356 & 0.345 & 0.293 \\
    & F1.5 & & 0.398 & 0.384 & 0.402 & 0.393 & 0.378 & 0.351 & 0.360 & 0.342 & 0.274 \\ %old model
    & F2.0 & & 0.439 & 0.420 & 0.430 & 0.415 &  0.396 & 0.362 & 0.372 & 0.348 & 0.270 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS18}}} 
    & F0.5 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F1.0 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F1.5 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F2.0 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{MO17}}} 
    & F0.5 & & 0.866 & 0.900 & 0.918 & 0.930 & 0.943 & 0.948 & 0.951 & 0.954 & 0.948 \\
    & F1.0 & & 0.907 & 0.928 & 0.936 & 0.941 & 0.944 & 0.942 & 0.938 & 0.932 & 0.902 \\
    & F1.5 & & 0.936 & 0.947 & 0.949 & 0.948 & 0.945 & 0.940 & 0.930 & 0.919 & 0.876 \\ %old model
    & F2.0 & & 0.954 & 0.959 & 0.957 & 0.953 &  0.946 & 0.939 & 0.926 & 0.913 & 0.862 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{PO18}}} 
    & F0.5 & & 0.610 & 0.630 & 0.639 & 0.647 & 0.664 & 0.656 & 0.663 & 0.657 & 0.651 \\
    & F1.0 & & 0.610 & 0.619 & 0.622 & 0.624 & 0.656 & 0.629 & 0.625 & 0.608 & 0.586 \\
    & F1.5 & & 0.622 & 0.623 & 0.623 & 0.620 & 0.660 & 0.623 & 0.612 & 0.589 & 0.559 \\ %old model
    & F2.0 & & 0.633 & 0.629 & 0.627 & 0.621 & 0.665 & 0.623 & 0.607 & 0.582 & 0.547 \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/supplementary_data/multiclass_tversky_fmeasures_stderr.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY}
    \toprule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{BR18}}} 
    & F0.5 & & 0.739 & 0.806 & 0.841 & 0.853 & 0.878 & 0.890 & 0.896 & 0.894 & 0.879 \\
    & F1.0 & & 0.801 & 0.844 & 0.859 & 0.863 & 0.870 & 0.867 & 0.857 & 0.831 & 0.787 \\
    & F1.5 & & 0.850 & 0.874 & 0.875 & 0.873 & 0.867 & 0.855 & 0.837 & 0.798 & 0.741 \\ %old model
    & F2.0 & & 0.882 & 0.893 & 0.885 & 0.880 &  0.867 & 0.850 & 0.827 & 0.782 & 0.719 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS17}}} 
    & F0.5 & & 0.316 & 0.318 & 0.358 & 0.372 & 0.368 & 0.367 & 0.387 & 0.382 & 0.363 \\
    & F1.0 & & 0.352 & 0.345 & 0.374 & 0.374 & 0.362 & 0.346 & 0.356 & 0.345 & 0.293 \\
    & F1.5 & & 0.398 & 0.384 & 0.402 & 0.393 & 0.378 & 0.351 & 0.360 & 0.342 & 0.274 \\ %old model
    & F2.0 & & 0.439 & 0.420 & 0.430 & 0.415 &  0.396 & 0.362 & 0.372 & 0.348 & 0.270 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS18}}} 
    & F0.5 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F1.0 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F1.5 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F2.0 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{MO17}}} 
    & F0.5 & & 0.866 & 0.900 & 0.918 & 0.930 & 0.943 & 0.948 & 0.951 & 0.954 & 0.948 \\
    & F1.0 & & 0.907 & 0.928 & 0.936 & 0.941 & 0.944 & 0.942 & 0.938 & 0.932 & 0.902 \\
    & F1.5 & & 0.936 & 0.947 & 0.949 & 0.948 & 0.945 & 0.940 & 0.930 & 0.919 & 0.876 \\ %old model
    & F2.0 & & 0.954 & 0.959 & 0.957 & 0.953 &  0.946 & 0.939 & 0.926 & 0.913 & 0.862 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{PO18}}} 
    & F0.5 & & 0.610 & 0.630 & 0.639 & 0.647 & 0.664 & 0.656 & 0.663 & 0.657 & 0.651 \\
    & F1.0 & & 0.610 & 0.619 & 0.622 & 0.624 & 0.656 & 0.629 & 0.625 & 0.608 & 0.586 \\
    & F1.5 & & 0.622 & 0.623 & 0.623 & 0.620 & 0.660 & 0.623 & 0.612 & 0.589 & 0.559 \\ %old model
    & F2.0 & & 0.633 & 0.629 & 0.627 & 0.621 & 0.665 & 0.623 & 0.607 & 0.582 & 0.547 \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/supplementary_data/multiclass_tversky_stderr.tex <==
% Results for new model:
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Type & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & 0.75/0.75 & 1.0/1.0\\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Dice}}} 
&All &        &        0.009 &        0.009 &        0.009 &        0.009 & 0.010 &        0.010 &        0.010 &        0.010 &        0.010 &        0.010 & 0.010 \\
&WT &        &        0.007 &        0.007 &        0.006 &        0.007 & 0.007 &        0.007 &        0.007 &        0.007 &        0.008 &        0.007 & 0.007 \\
&TC &        &        0.012 &        0.011 &        0.012 &        0.012 & 0.013 &        0.013 &        0.014 &        0.014 &        0.014 &        0.013 & 0.014 \\
&ET &        &        0.016 &        0.016 &        0.017 &        0.017 & 0.017 &        0.017 &        0.018 &        0.017 &        0.016 &        0.018 & 0.017 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
&All &        &        0.008 &        0.009 &        0.009 &        0.010 & 0.010 &        0.010 &        0.010 &        0.010 &        0.010 &        0.010 & 0.010 \\
&WT &        &        0.009 &        0.008 &        0.008 &        0.008 & 0.009 &        0.008 &        0.009 &        0.009 &        0.010 &        0.008 & 0.008 \\
&TC &        &        0.012 &        0.012 &        0.013 &        0.013 & 0.014 &        0.014 &        0.014 &        0.014 &        0.014 &        0.014 & 0.014 \\
&ET &        &        0.014 &        0.014 &        0.015 &        0.016 & 0.016 &        0.016 &        0.016 &        0.015 &        0.015 &        0.016 & 0.016 \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/supplementary_data/tversky_fmeasures.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Measure & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & 0.75/0.75 & 1.0/1.0 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{BR18}}} 
    & F0.5 & & \textit{0.739} & 0.806 & 0.841 & 0.853 & 0.878 & 0.890 & \cellcolor{gray!50}0.896 & \cellcolor{gray!50}0.894 & 0.879 &  0.878 & 0.877 \\
    & F1.0 & & 0.801 & 0.844 & 0.859 & 0.863 & \cellcolor{gray!50}0.870 & \cellcolor{gray!50}0.867 & 0.857 & 0.831 & \textit{0.787} &  \cellcolor{gray!50}0.871 & \cellcolor{gray!50}0.868 \\
    & F1.5 & & 0.850 & \cellcolor{gray!50}0.874 & \cellcolor{gray!50}0.875 & \cellcolor{gray!50}0.873 & 0.867 & 0.855 & 0.837 & 0.798 & \textit{0.741} &  0.869 & 0.865 \\
    & F2.0 & & 0.882 & \cellcolor{gray!50}0.893 & 0.885 & 0.880 & 0.867 & 0.850 & 0.827 & 0.782 & \textit{0.719} &  0.869 & 0.865 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS17}}} 
    & F0.5 & & 0.316 & 0.318 & \cellcolor{gray!50}0.358 & \cellcolor{gray!50}0.372 & \cellcolor{gray!50}0.368 & \cellcolor{gray!50}0.367 & \cellcolor{gray!50}0.387 & \cellcolor{gray!50}0.382 & \cellcolor{gray!50}0.363 &  0.367 & 0.362 \\
    & F1.0 & & \cellcolor{gray!50}0.352 & 0.345 & \cellcolor{gray!50}0.374 & \cellcolor{gray!50}0.374 & \cellcolor{gray!50}0.362 & 0.346 & \cellcolor{gray!50}0.356 & \cellcolor{gray!50}0.345 & 0.293 &  \cellcolor{gray!50}0.371 & \cellcolor{gray!50}0.363 \\
    & F1.5 & & \cellcolor{gray!50}0.398 & \cellcolor{gray!50}0.384 & \cellcolor{gray!50}0.402 & \cellcolor{gray!50}0.393 & \cellcolor{gray!50}0.378 & 0.351 & 0.360 & 0.342 & \textit{0.274} &  \cellcolor{gray!50}0.394 & \cellcolor{gray!50}0.384 \\
    & F2.0 & & \cellcolor{gray!50}0.439 & \cellcolor{gray!50}0.420 & \cellcolor{gray!50}0.430 & \cellcolor{gray!50}0.415 & \cellcolor{gray!50}0.396 & 0.362 & 0.372 & 0.348 & \textit{0.270} &  \cellcolor{gray!50}0.419 & \cellcolor{gray!50}0.408 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS18}}} 
    & F0.5 & & \textit{0.411} & 0.468 & 0.495 & 0.516 & \cellcolor{gray!50}0.528 & 0.528 & \cellcolor{gray!50}0.539 & \cellcolor{gray!50}0.543 & \cellcolor{gray!50}0.530 &  0.521 & 0.520 \\
    & F1.0 & & 0.481 & 0.522 & 0.533 & \cellcolor{gray!50}0.540 & \cellcolor{gray!50}0.538 & \cellcolor{gray!50}0.527 & 0.519 & 0.490 & \textit{0.445} &  0.528 & 0.528 \\
    & F1.5 & & 0.551 & \cellcolor{gray!50}0.573 & \cellcolor{gray!50}0.571 & \cellcolor{gray!50}0.568 & 0.555 & 0.537 & 0.517 & 0.470 & \textit{0.413} &  0.544 & 0.544 \\
    & F2.0 & & \cellcolor{gray!50}0.607 & \cellcolor{gray!50}0.612 & 0.600 & 0.590 & 0.569 & 0.547 & 0.520 & 0.464 & \textit{0.399} &  0.558 & 0.558 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{MO17}}} 
    & F0.5 & & \textit{0.866} & 0.900 & 0.918 & 0.930 & 0.943 & 0.948 & 0.951 & \cellcolor{gray!50}0.954 & 0.948 &  0.943 & 0.942 \\
    & F1.0 & & 0.907 & 0.928 & 0.936 & 0.941 & \cellcolor{gray!50}0.944 & \cellcolor{gray!50}0.942 & 0.938 & 0.932 & 0.902 &  \cellcolor{gray!50}0.944 & \cellcolor{gray!50}0.942 \\
    & F1.5 & & 0.936 & 0.947 & \cellcolor{gray!50}0.949 & \cellcolor{gray!50}0.948 & 0.945 & 0.940 & 0.930 & 0.919 & \textit{0.876} &  0.945 & 0.944 \\
    & F2.0 & & 0.954 & \cellcolor{gray!50}0.959 & 0.957 & 0.953 & 0.946 & 0.939 & 0.926 & 0.913 & \textit{0.862} &  0.946 & 0.945 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{PO18}}} 
    & F0.5 & & \textit{0.588} & 0.609 & 0.625 & 0.644 & \cellcolor{gray!50}0.664 & \cellcolor{gray!50}0.664 & \cellcolor{gray!50}0.671 & \cellcolor{gray!50}0.669 & \cellcolor{gray!50}0.664 & 0.656 & 0.657 \\
    & F1.0 & & 0.614 & 0.628 & 0.637 & 0.647 & \cellcolor{gray!50}0.656 & \cellcolor{gray!50}0.650 & 0.647 & 0.633 & 0.611 & 0.646 & \cellcolor{gray!50}0.651 \\
    & F1.5 & & 0.643 & 0.651 & \cellcolor{gray!50}0.654 & \cellcolor{gray!50}0.658 & \cellcolor{gray!50}0.660 & 0.651 & 0.641 & 0.620 & \textit{0.591} & 0.650 & \cellcolor{gray!50}0.656 \\
    & F2.0 & & \cellcolor{gray!50}0.665 & \cellcolor{gray!50}0.669 & \cellcolor{gray!50}0.668 & \cellcolor{gray!50}0.668 & \cellcolor{gray!50}0.665 & 0.655 & 0.640 & 0.616 & \textit{0.582} & 0.655 & \cellcolor{gray!50}0.662 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{WM17}}} 
    & F0.5 & & \textit{0.498} & 0.592 & 0.659 & 0.690 & 0.724 & 0.742 & \cellcolor{gray!50}0.761 & \cellcolor{gray!50}0.759 & 0.720 &  0.723 & 0.730 \\
    & F1.0 & & 0.581 & 0.649 & 0.689 & 0.700 & \cellcolor{gray!50}0.712 & 0.706 & 0.693 & 0.660 & 0.565 &  \cellcolor{gray!50}0.712 & \cellcolor{gray!50}0.712 \\
    & F1.5 & & 0.657 & 0.700 & \cellcolor{gray!50}0.718 & 0.713 & \cellcolor{gray!50}0.711 & 0.692 & 0.660 & 0.615 & \textit{0.501} &  0.712 & 0.708 \\
    & F2.0 & & 0.714 & \cellcolor{gray!50}0.736 & \cellcolor{gray!50}0.739 & 0.724 & 0.713 & 0.686 & 0.645 & 0.593 & \textit{0.472} &  0.714 & 0.708 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{WM17\textsuperscript{DM}}}} 
    & F0.5 & & \textit{0.521} & 0.617 & 0.671 & 0.709 & 0.736 & \cellcolor{gray!50}0.758 & \cellcolor{gray!50}0.759 & \cellcolor{gray!50}0.752 & 0.647 &  0.731 & 0.736 \\
    & F1.0 & & 0.599 & 0.668 & 0.696 & 0.709 & \cellcolor{gray!50}0.717 & 0.706 & 0.675 & 0.628 & \textit{0.496} &  0.706 & \cellcolor{gray!50}0.714 \\
    & F1.5 & & 0.670 & \cellcolor{gray!50}0.713 & \cellcolor{gray!50}0.722 & \cellcolor{gray!50}0.717 & 0.712 & 0.682 & 0.636 & 0.574 & \textit{0.436} &  0.697 & 0.707 \\
    & F2.0 & & 0.721 & \cellcolor{gray!50}0.744 & \cellcolor{gray!50}0.739 & 0.723 & 0.712 & 0.672 & 0.618 & 0.548 & \textit{0.409} &  0.695 & 0.706 \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/supplementary_data/tversky_fmeasures_stderr.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Measure & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & 0.75/0.75 & 1.0/1.0 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{BR18}}} 
    & F0.5 & & 0.008 & 0.007 & 0.007 & 0.007 & 0.006 & 0.005 & 0.006 & 0.006 & 0.006 &  0.006 & 0.007 \\
    & F1.0 & & 0.007 & 0.006 & 0.006 & 0.006 & 0.006 & 0.006 & 0.007 & 0.007 & 0.008 &  0.006 & 0.007 \\
    & F1.5 & & 0.006 & 0.005 & 0.006 & 0.006 & 0.006 & 0.006 & 0.007 & 0.008 & 0.009 &  0.007 & 0.007 \\
    & F2.0 & & 0.005 & 0.005 & 0.006 & 0.007 & 0.007 & 0.007 & 0.008 & 0.009 & 0.009 &  0.007 & 0.007 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS17}}} 
    & F0.5 & & 0.034 & 0.035 & 0.039 & 0.040 & 0.037 & 0.038 & 0.038 & 0.037 & 0.036 &  0.036 & 0.037 \\
    & F1.0 & & 0.036 & 0.035 & 0.037 & 0.037 & 0.034 & 0.034 & 0.033 & 0.034 & 0.031 &  0.033 & 0.035 \\
    & F1.5 & & 0.037 & 0.036 & 0.036 & 0.036 & 0.034 & 0.033 & 0.032 & 0.034 & 0.030 &  0.033 & 0.035 \\
    & F2.0 & & 0.039 & 0.037 & 0.036 & 0.037 & 0.034 & 0.034 & 0.032 & 0.035 & 0.030 &  0.034 & 0.036 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS18}}} 
    & F0.5 & & 0.024 & 0.026 & 0.026 & 0.027 & 0.028 & 0.028 & 0.029 & 0.029 & 0.030 &  0.028 & 0.028 \\
    & F1.0 & & 0.025 & 0.026 & 0.026 & 0.026 & 0.027 & 0.027 & 0.027 & 0.027 & 0.027 &  0.027 & 0.027 \\
    & F1.5 & & 0.025 & 0.026 & 0.026 & 0.026 & 0.027 & 0.027 & 0.027 & 0.026 & 0.026 &  0.027 & 0.027 \\
    & F2.0 & & 0.026 & 0.026 & 0.027 & 0.026 & 0.027 & 0.027 & 0.027 & 0.026 & 0.025 &  0.027 & 0.027 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{MO17}}} 
    & F0.5 & & 0.004 & 0.004 & 0.004 & 0.003 & 0.003 & 0.003 & 0.002 & 0.003 & 0.002 &  0.003 & 0.003 \\
    & F1.0 & & 0.003 & 0.003 & 0.003 & 0.003 & 0.003 & 0.003 & 0.002 & 0.003 & 0.003 &  0.002 & 0.003 \\
    & F1.5 & & 0.002 & 0.002 & 0.002 & 0.002 & 0.002 & 0.003 & 0.002 & 0.003 & 0.003 &  0.002 & 0.003 \\
    & F2.0 & & 0.002 & 0.002 & 0.002 & 0.002 & 0.002 & 0.003 & 0.002 & 0.003 & 0.004 &  0.002 & 0.003 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{PO18}}} 
    & F0.5 & & 0.009 & 0.009 & 0.009 & 0.009 & 0.009 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.009 \\
    & F1.0 & & 0.009 & 0.009 & 0.009 & 0.009 & 0.009 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 \\
    & F1.5 & & 0.009 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 \\
    & F2.0 & & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{WM17}}} 
    & F0.5 & & 0.019 & 0.019 & 0.018 & 0.020 & 0.018 & 0.019 & 0.017 & 0.018 & 0.020 &  0.020 & 0.019 \\
    & F1.0 & & 0.018 & 0.018 & 0.018 & 0.018 & 0.019 & 0.020 & 0.019 & 0.020 & 0.021 &  0.019 & 0.020 \\
    & F1.5 & & 0.018 & 0.019 & 0.018 & 0.019 & 0.020 & 0.021 & 0.020 & 0.021 & 0.021 &  0.019 & 0.021 \\
    & F2.0 & & 0.017 & 0.019 & 0.019 & 0.019 & 0.021 & 0.021 & 0.021 & 0.021 & 0.020 &  0.020 & 0.021 \\ 
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{WM17\textsuperscript{DM}}}} 
    & F0.5 & & 0.018 & 0.017 & 0.018 & 0.017 & 0.017 & 0.018 & 0.019 & 0.020 & 0.032 &  0.018 & 0.018 \\
    & F1.0 & & 0.018 & 0.018 & 0.018 & 0.018 & 0.019 & 0.020 & 0.022 & 0.023 & 0.030 &  0.020 & 0.020 \\
    & F1.5 & & 0.018 & 0.018 & 0.020 & 0.020 & 0.020 & 0.022 & 0.023 & 0.024 & 0.029 &  0.021 & 0.022 \\
    & F2.0 & & 0.018 & 0.019 & 0.021 & 0.021 & 0.021 & 0.022 & 0.024 & 0.024 & 0.028 &  0.022 & 0.023 \\
    \bottomrule
\end{tabularx}


==> TMI - Dice/supplementary_data/tversky_stderr.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & 0.75/0.75 & 1.0/1.0 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    &BR18 &        &        0.007 &        0.006 &        0.006 &        0.006 & 0.006 &        0.006 &        0.007 &        0.007 &        0.008 &        0.006 & 0.007 \\
    &IS17 &        &        0.036 &        0.035 &        0.037 &        0.037 & 0.034 &        0.034 &        0.033 &        0.034 &        0.031 &        0.033 & 0.035 \\
    &IS18 &        &        0.025 &        0.026 &        0.026 &        0.026 & 0.027 &        0.027 &        0.027 &        0.027 &        0.027 &        0.027 & 0.027 \\
    &MO18 &        &        0.003 &        0.003 &        0.003 &        0.003 & 0.003 &        0.003 &        0.002 &        0.003 &        0.003 &        0.002 & 0.003 \\
    &PO18 &        &        0.009 &        0.009 &        0.009 &        0.009 & 0.009 &        0.010 &        0.010 &        0.010 &        0.010 &          0.010 & 0.010 \\
    &WM17 &        &        0.018 &        0.018 &        0.018 &        0.018 & 0.019 &        0.020 &        0.019 &        0.020 &        0.021 &        0.019 & 0.020 \\
    &WM17\textsuperscript{DM} &        &        0.018 &        0.018 &        0.018 &        0.018 & 0.019 &        0.020 &        0.022 &        0.023 &        0.030 &        0.020 & 0.020 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    &BR18 &        &        0.008 &        0.007 &        0.008 &        0.008 & 0.008 &        0.007 &        0.008 &        0.009 &        0.010 &        0.008 & 0.008 \\
    &IS17 &        &        0.028 &        0.027 &        0.028 &        0.029 & 0.027 &        0.026 &        0.025 &        0.025 &        0.022 &        0.026 & 0.028 \\
    &IS18 &        &        0.022 &        0.023 &        0.023 &        0.023 & 0.023 &        0.023 &        0.023 &        0.023 &        0.022 &        0.024 & 0.024 \\
    &MO18 &        &        0.004 &        0.004 &        0.004 &        0.004 & 0.004 &        0.004 &        0.003 &        0.004 &        0.004 &        0.003 & 0.004 \\
    &PO18 &        &        0.008 &        0.009 &        0.009 &        0.009 & 0.009 &        0.009 &        0.009 &        0.009 &        0.009 &          0.009 & 0.009 \\
    &WM17 &        &        0.017 &        0.019 &        0.019 &        0.021 & 0.021 &        0.021 &        0.021 &        0.021 &        0.019 &        0.021 & 0.022 \\
    &WM17\textsuperscript{DM} &        &        0.017 &        0.018 &        0.020 &        0.021 & 0.021 &        0.022 &        0.023 &        0.023 &        0.026 &        0.022 & 0.022 \\
    \bottomrule
\end{tabularx}

==> TMI - Dice/tversky/tversky_results.tex <==
% % Results for old model:
% \begin{tabularx}{\linewidth}{lsXYYYYYYYYY}
%     \toprule
%     & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice score}}} 
%     & BR18 & & 0.740 & 0.791 & 0.811 & 0.820 & 0.818 & 0.823 & 0.808 & 0.790 & 0.735 \\
%     & IS17 & & 0.315 & 0.323 & 0.337 & 0.326 & 0.320 & 0.312 & 0.306 & 0.301 & 0.258 \\
%     & IS18 & & 0.475 & 0.515 & 0.526 & 0.540 & 0.536 & 0.527 & 0.518 & 0.490 & 0.445 \\
%     & MO17 & & 0.893 & 0.920 & 0.928 & 0.929 & 0.930 & 0.930 & 0.928 & 0.915 & 0.890 \\
%     & PO18 & & 0.610 & 0.619 & 0.623 & 0.624 & 0.656 & 0.629 & 0.625 & 0.609 & 0.586 \\ %old model == new model
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard index}}}
%     & BR18 & & 0.590 & 0.662 & 0.693 & 0.707 & 0.703 & 0.712 & 0.694 & 0.668 & 0.603 \\
%     & IS17 & & 0.213 & 0.221 & 0.229 & 0.220 & 0.214 & 0.208 & 0.204 & 0.199 & 0.168 \\
%     & IS18 & & 0.345 & 0.384 & 0.396 & 0.407 & 0.404 & 0.398 & 0.390 & 0.361 & 0.321 \\
%     & MO17 & & 0.813 & 0.858 & 0.870 & 0.872 & 0.875 & 0.873 & 0.870 & 0.848 & 0.806 \\
%     & PO18 & & 0.505 & 0.518 & 0.524 & 0.527 & 0.559 & 0.534 & 0.530 & 0.515 & 0.491 \\ %old model == new model
%     \bottomrule
% \end{tabularx}

% Results for new model:
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & \review{0.75/0.75} & \review{1.0/1.0} \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    &BR18 &        &        0.801 &        0.844 &        0.859 &        0.863 & \cellcolor{gray!50}0.870 &   \cellcolor{gray!50}     0.867 &        0.857 &        0.831 &        \textit{0.787} &     \cellcolor{gray!50}   \review{0.871} & \cellcolor{gray!50}\review{0.868} \\
    &IS17 &        &    \cellcolor{gray!50}    0.352 &        0.345 &    \cellcolor{gray!50}    0.374 &   \cellcolor{gray!50}     0.374 &\cellcolor{gray!50} 0.362 &        0.346 &    \cellcolor{gray!50}    0.356 &    \cellcolor{gray!50}    0.345 &        0.293 &      \cellcolor{gray!50}  \review{0.371} & \cellcolor{gray!50}\review{0.363} \\
    &IS18 &        &        0.481 &        0.522 &        0.533 &     \cellcolor{gray!50}   0.540 & \cellcolor{gray!50}0.538 &    \cellcolor{gray!50}    0.527 &        0.519 &        0.490 &        \textit{0.445} &        \review{0.528} & \review{0.528} \\
    &MO18 &        &        0.907 &        0.928 &        0.936 &        0.941 & \cellcolor{gray!50}0.944 &    \cellcolor{gray!50}    0.942 &        0.938 &        0.932 &        0.902 &    \cellcolor{gray!50}   \review{0.944} & \cellcolor{gray!50}\review{0.942} \\
    &PO18 &        &        0.615 &        0.628 &        0.638 &        0.647 & \cellcolor{gray!50}0.656 &   \cellcolor{gray!50}     0.651 &        0.647 &        0.633 &        0.611 &          \review{0.646} & \cellcolor{gray!50}\review{0.651} \\
    &\review{WM17} &        &        \review{0.581} &        \review{0.649} &        \review{0.689} &        \review{0.700} & \cellcolor{gray!50}\review{0.712} &        \review{0.706} &        \review{0.693} &        \review{0.660} &        \review{0.565} &      \cellcolor{gray!50}  \review{0.712} & \cellcolor{gray!50}\review{0.712} \\
    &\review{WM17\textsuperscript{DM}} &        &        \review{0.599} &        \review{0.668} &        \review{0.696} &        \review{0.709} & \cellcolor{gray!50}\review{0.717} &        \review{0.706} &        \review{0.675} &        \review{0.628} &        \review{\textit{0.496}} &        \review{0.706} & \cellcolor{gray!50}\review{0.714} \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    &BR18 &        &        0.680 &        0.740 &        0.765 &        0.772 & \cellcolor{gray!50}0.780 &        0.775 &        0.764 &        0.726 &        \textit{0.666} &     \cellcolor{gray!50}   \review{0.783} & \cellcolor{gray!50}\review{0.780} \\
    &IS17 &        &        0.239 &        0.232 &     \cellcolor{gray!50}   0.257 &   \cellcolor{gray!50}     0.257 &\cellcolor{gray!50} 0.244 &        0.231 &    \cellcolor{gray!50}    0.238 &    \cellcolor{gray!50}    0.230 &        \textit{0.188} &      \cellcolor{gray!50} \review{0.250} &\cellcolor{gray!50} \review{0.246} \\
    &IS18 &        &        0.349 &        0.389 &     \cellcolor{gray!50}   0.401 &    \cellcolor{gray!50}    0.407 & \cellcolor{gray!50}0.407 &        0.398 &        0.390 &        0.361 &      \textit{0.321} &        \review{0.399} & \review{0.399} \\
    &MO18 &        &        0.834 &        0.870 &        0.884 &        0.892 & \cellcolor{gray!50}0.897 &    \cellcolor{gray!50}    0.895 &        0.886 &        0.876 &        0.826 &    \cellcolor{gray!50}    \review{0.896} & \cellcolor{gray!50}\review{0.896} \\
    &PO18 &        &        0.504 &        0.523 &        0.536 &        0.548 &\cellcolor{gray!50} 0.559 &   \cellcolor{gray!50}     0.556 &   \cellcolor{gray!50}     0.554 &        0.539 &        0.511 &          \review{0.550} & \cellcolor{gray!50}\review{0.554} \\
    &\review{WM17} &        &        \review{0.422} &        \review{0.496} &        \review{0.541} &        \review{0.556} &\cellcolor{gray!50} \review{0.571} &        \review{0.565} &        \review{0.548} &        \review{0.510} &        \review{0.410} &      \cellcolor{gray!50}  \review{0.571} & \cellcolor{gray!50}\review{0.573} \\
    &\review{WM17\textsuperscript{DM}} &        &        \review{0.441} &        \review{0.516} &        \review{0.551} &        \review{0.566} & \cellcolor{gray!50}\review{0.577} &        \review{0.566} &        \review{0.532} &        \review{0.481} &        \review{\textit{0.360}} &        \review{0.565} & \cellcolor{gray!50}\review{0.576} \\
    \bottomrule
\end{tabularx}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> significances_tbl.tex <==
% \begin{tabularx}{\linewidth}{ll|Y|Y|Y|Y|Y}
% \toprule
%      & Loss &   CE &  wCE & DICE & JACC & LOVA \\
% Dataset & Loss &      &      &      &      &      \\
% \midrule
% MO18 & CE &  000 &  111 &  000 &  000 &  000 \\
%      & wCE &  000 &  000 &  000 &  000 &  000 \\
%      & DICE &  011 &  111 &  000 &  000 &  000 \\
%      & JACC &  000 &  111 &  000 &  000 &  000 \\
%      & LOVA &  011 &  111 &  000 &  000 &  000 \\
% BR18 & CE &  000 &  111 &  000 &  000 &  000 \\
%      & wCE &  000 &  000 &  000 &  000 &  000 \\
%      & DICE &  111 &  111 &  000 &  000 &  000 \\
%      & JACC &  111 &  111 &  100 &  000 &  000 \\
%      & LOVA &  111 &  111 &  111 &  010 &  000 \\
% IS17 & CE &  000 &  100 &  100 &  100 &  100 \\
%      & wCE &  011 &  000 &  000 &  000 &  000 \\
%      & DICE &  011 &  010 &  000 &  000 &  011 \\
%      & JACC &  011 &  100 &  100 &  000 &  000 \\
%      & LOVA &  011 &  000 &  000 &  000 &  000 \\
% IS18 & CE &  000 &  100 &  100 &  100 &  100 \\
%      & wCE &  000 &  000 &  000 &  000 &  000 \\
%      & DICE &  011 &  111 &  000 &  011 &  011 \\
%      & JACC &  011 &  111 &  000 &  000 &  011 \\
%      & LOVA &  011 &  111 &  000 &  000 &  000 \\
% PO18 & CE &  000 &  111 &  000 &  100 &  000 \\
%      & wCE &  000 &  000 &  000 &  000 &  000 \\
%      & DICE &  011 &  111 &  000 &  000 &  000 \\
%      & JACC &  011 &  111 &  000 &  000 &  000 \\
%      & LOVA &  011 &  111 &  000 &  000 &  000 \\
% \bottomrule
% \end{tabularx}

\begin{tabularx}{\linewidth}{ll|Y|Y|Y|Y|Y}
\toprule
     & Train loss: &   CE &  wCE & sDice & sJaccard & Lov\`{a}sz \\
Dataset: & Train loss: &      &      &      &      &      \\
\midrule
BR18 & CE &  00 &  11 &  00 &  00 &  00 \\
     & wCE &  00 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  11 &  00 &  00 &  00 \\
     & sJaccard &  11 &  11 &  00 &  00 &  00 \\
     & Lov\`{a}sz &  11 &  11 &  11 &  10 &  00 \\
IS17 & CE &  00 &  00 &  00 &  00 &  00 \\
     & wCE &  11 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  10 &  00 &  00 &  11 \\
     & sJaccard &  11 &  00 &  00 &  00 &  00 \\
     & Lov\`{a}sz &  11 &  00 &  00 &  00 &  00 \\
IS18 & CE &  00 &  00 &  00 &  00 &  00 \\
     & wCE &  00 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  11 &  00 &  11 &  11 \\
     & sJaccard &  11 &  11 &  00 &  00 &  11 \\
     & Lov\`{a}sz &  11 &  11 &  00 &  00 &  00 \\
MO17 & CE &  00 &  11 &  00 &  00 &  00 \\
     & wCE &  00 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  11 &  00 &  00 &  00 \\
     & sJaccard &  00 &  11 &  00 &  00 &  00 \\
     & Lov\`{a}sz &  11 &  11 &  00 &  00 &  00 \\
PO18 & CE &  00 &  11 &  00 &  00 &  00 \\
     & wCE &  00 &  00 &  00 &  00 &  00 \\
     & sDice &  11 &  11 &  00 &  00 &  00 \\
     & sJaccard &  11 &  11 &  00 &  00 &  00 \\
     & Lov\`{a}sz &  11 &  11 &  00 &  00 &  00 \\
\bottomrule
\end{tabularx}

==> supplementary_data/crop_results_stderr.tex <==
\begin{tabularx}{\linewidth}{llXYYYYY}
    \toprule
         & Loss & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{Dataset} $\rightarrow$}} & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\
    \midrule
\parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Dice}}}
      & CE    & &  0.010 &  0.009 &  0.009 &  0.009 &  0.008 \\
      & sDice & &  0.009 &  0.009 &  0.009 &  0.008 &  0.008 \\
    \midrule
    \parbox[t]{3mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Jacc.}}}
      & CE    & &  0.009 &  0.009 &  0.009 &  0.009 &  0.009 \\
      & sDice & &  0.009 &  0.009 &  0.009 &  0.008 &  0.008 \\
         
    \bottomrule
\end{tabularx}

==> supplementary_data/empirical_results_stderr.tex <==
% Std Error
\begin{tabularx}{\linewidth}{lsXYYYYY}
    \toprule
    & & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{group} $\rightarrow$}} & \multicolumn{2}{c}{CE-based} & \multicolumn{3}{c}{Metric-sensitive} \\
    \midrule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    & BR18 &        & 0.007 & 0.008 & 0.006 & 0.007 & 0.006 \\
    & IS17 &        & 0.039 & 0.039 & 0.034 & 0.035 & 0.038 \\
    & IS18 &        & 0.029 & 0.026 & 0.027 & 0.027 & 0.028 \\
    & MO18 &        & 0.003 & 0.005 & 0.003 & 0.003 & 0.002 \\
    & PO18 &        & 0.010 & 0.009 & 0.009 & 0.010 & 0.010 \\
    & WM17 &        & 0.023 & 0.029 & 0.019 & 0.020 & 0.020 \\
    & WM17\textsuperscript{DM} &        & 0.022 & 0.034 & 0.019 & 0.020 & 0.021 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    & BR18 &        & 0.009 & 0.009 & 0.008 & 0.008 & 0.008 \\
    & IS17 &        & 0.029 & 0.030 & 0.027 & 0.028 & 0.029 \\
    & IS18 &        & 0.025 & 0.023 & 0.023 & 0.024 & 0.024 \\
    & MO18 &        & 0.004 & 0.006 & 0.004 & 0.004 & 0.004 \\
    & PO18 &        & 0.009 & 0.008 & 0.009 & 0.009 & 0.009 \\
    & WM17 &        & 0.024 & 0.025 & 0.021 & 0.022 & 0.022 \\
    & WM17\textsuperscript{DM} &        & 0.024 & 0.029 & 0.021 & 0.022 & 0.023 \\
    \bottomrule
\end{tabularx}

% IQR
% \begin{tabularx}{\linewidth}{lsXYYYYY}
%     \toprule
%     & & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{group} $\rightarrow$}} & \multicolumn{2}{c}{CE-based} & \multicolumn{3}{c}{Metric-sensitive} \\
%     \midrule
%     & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice}}} 
%     &BR18 &        & 0.097 & 0.134 & 0.081 & 0.083 & 0.084 \\
%     &IS17 &        & 0.466 & 0.473 & 0.335 & 0.357 & 0.421 \\
%     &IS18 &        & 0.479 & 0.322 & 0.324 & 0.318 & 0.379 \\
%     &MO18 &        & 0.029 & 0.054 & 0.031 & 0.031 & 0.029 \\
%     &PO18 &        & 0.462 & 0.385 & 0.389 & 0.395 & 0.417 \\
%     &WM17 &        & 0.228 & 0.291 & 0.186 & 0.186 & 0.176 \\
%     &WM17\textsuperscript{DM} &        & 0.238 & 0.456 & 0.195 & 0.203 & 0.215 \\   
%     \midrule
%     \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
%     &BR18 &        & 0.152 & 0.197 & 0.130 & 0.135 & 0.137 \\
%     &IS17 &        & 0.304 & 0.344 & 0.251 & 0.270 & 0.309 \\
%     &IS18 &        & 0.422 & 0.295 & 0.317 & 0.310 & 0.356 \\
%     &MO18 &        & 0.053 & 0.093 & 0.056 & 0.057 & 0.053 \\
%     &PO18 &        & 0.537 & 0.426 & 0.472 & 0.477 & 0.500 \\
%     &WM17 &        & 0.269 & 0.259 & 0.229 & 0.231 & 0.215 \\
%     &WM17\textsuperscript{DM} &        & 0.280 & 0.354 & 0.243 & 0.252 & 0.264 \\
%     \bottomrule
% \end{tabularx}


==> supplementary_data/l1vsl2_stderr.tex <==
\begin{tabularx}{\linewidth}{llXYYYYYYY}
    \toprule
         & Loss & \multicolumn{1}{l}{\lapbox[0.5\width]{0.5em}{\emph{Data} $\rightarrow$}} & BR18 & IS17 & IS18 & MO17 & PO18 & WM17 & WM17\textsuperscript{DM} \\
    \midrule
    \parbox[t]{1mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Dice}}}
      & $L^1$   & &  0.006 &  0.034 &  0.027 &  0.003 &  0.009 & 0.019 & 0.019 \\
      & $L^2$   & &  0.006 &  0.037 &  0.027 &  0.002 &  0.011   & 0.019 & 0.020\\
    \midrule
    \parbox[t]{1mm}{\centering\multirow{2}{*}{\rotatebox[origin=c]{90}{Jacc.}}}
      & $L^1$   & &  0.008 &  0.027 &  0.023 &  0.004 &  0.009 & 0.021 & 0.021 \\
      & $L^2$   & &  0.008 &  0.029 &  0.024 &  0.004 &  0.011   & 0.021 & 0.023 \\
         
    \bottomrule
\end{tabularx}

==> supplementary_data/multiclass_results_stderr.tex <==
\begin{tabularx}{\linewidth}{llXYY|YYY}
    \toprule
    & & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{group} $\rightarrow$}} & \multicolumn{2}{c}{CE-based} & \multicolumn{3}{c}{Metric-sensitive} \\
    \midrule
    & Type & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{loss} $\rightarrow$}} & CE & wCE & sDice & sJaccard & Lov\'{a}sz \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    & All & & 0.011 & 0.012 & 0.010 & 0.010 & 0.010 \\
    & WT  & & 0.008 & 0.009 & 0.007 & 0.007 & 0.007 \\
    & TC  & & 0.014 & 0.016 & 0.013 & 0.014 & 0.014 \\
    & ET  & & 0.020 & 0.019 & 0.017 & 0.017 & 0.018 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    & All    & & 0.010 & 0.012 & 0.010 & 0.010 & 0.010 \\
    & WT     & & 0.010 & 0.010 & 0.009 & 0.008 & 0.008 \\
    & TC     & & 0.013 & 0.016 & 0.014 & 0.014 & 0.014 \\
    & ET     & & 0.018 & 0.018 & 0.016 & 0.016 & 0.016 \\
    \bottomrule
\end{tabularx}

==> supplementary_data/multiclass_tversky_fmeasures.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY}
    \toprule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{BR18}}} 
    & F0.5 & & 0.739 & 0.806 & 0.841 & 0.853 & 0.878 & 0.890 & 0.896 & 0.894 & 0.879 \\
    & F1.0 & & 0.801 & 0.844 & 0.859 & 0.863 & 0.870 & 0.867 & 0.857 & 0.831 & 0.787 \\
    & F1.5 & & 0.850 & 0.874 & 0.875 & 0.873 & 0.867 & 0.855 & 0.837 & 0.798 & 0.741 \\ %old model
    & F2.0 & & 0.882 & 0.893 & 0.885 & 0.880 &  0.867 & 0.850 & 0.827 & 0.782 & 0.719 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS17}}} 
    & F0.5 & & 0.316 & 0.318 & 0.358 & 0.372 & 0.368 & 0.367 & 0.387 & 0.382 & 0.363 \\
    & F1.0 & & 0.352 & 0.345 & 0.374 & 0.374 & 0.362 & 0.346 & 0.356 & 0.345 & 0.293 \\
    & F1.5 & & 0.398 & 0.384 & 0.402 & 0.393 & 0.378 & 0.351 & 0.360 & 0.342 & 0.274 \\ %old model
    & F2.0 & & 0.439 & 0.420 & 0.430 & 0.415 &  0.396 & 0.362 & 0.372 & 0.348 & 0.270 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS18}}} 
    & F0.5 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F1.0 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F1.5 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F2.0 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{MO17}}} 
    & F0.5 & & 0.866 & 0.900 & 0.918 & 0.930 & 0.943 & 0.948 & 0.951 & 0.954 & 0.948 \\
    & F1.0 & & 0.907 & 0.928 & 0.936 & 0.941 & 0.944 & 0.942 & 0.938 & 0.932 & 0.902 \\
    & F1.5 & & 0.936 & 0.947 & 0.949 & 0.948 & 0.945 & 0.940 & 0.930 & 0.919 & 0.876 \\ %old model
    & F2.0 & & 0.954 & 0.959 & 0.957 & 0.953 &  0.946 & 0.939 & 0.926 & 0.913 & 0.862 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{PO18}}} 
    & F0.5 & & 0.610 & 0.630 & 0.639 & 0.647 & 0.664 & 0.656 & 0.663 & 0.657 & 0.651 \\
    & F1.0 & & 0.610 & 0.619 & 0.622 & 0.624 & 0.656 & 0.629 & 0.625 & 0.608 & 0.586 \\
    & F1.5 & & 0.622 & 0.623 & 0.623 & 0.620 & 0.660 & 0.623 & 0.612 & 0.589 & 0.559 \\ %old model
    & F2.0 & & 0.633 & 0.629 & 0.627 & 0.621 & 0.665 & 0.623 & 0.607 & 0.582 & 0.547 \\
    \bottomrule
\end{tabularx}

==> supplementary_data/multiclass_tversky_fmeasures_stderr.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY}
    \toprule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{BR18}}} 
    & F0.5 & & 0.739 & 0.806 & 0.841 & 0.853 & 0.878 & 0.890 & 0.896 & 0.894 & 0.879 \\
    & F1.0 & & 0.801 & 0.844 & 0.859 & 0.863 & 0.870 & 0.867 & 0.857 & 0.831 & 0.787 \\
    & F1.5 & & 0.850 & 0.874 & 0.875 & 0.873 & 0.867 & 0.855 & 0.837 & 0.798 & 0.741 \\ %old model
    & F2.0 & & 0.882 & 0.893 & 0.885 & 0.880 &  0.867 & 0.850 & 0.827 & 0.782 & 0.719 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS17}}} 
    & F0.5 & & 0.316 & 0.318 & 0.358 & 0.372 & 0.368 & 0.367 & 0.387 & 0.382 & 0.363 \\
    & F1.0 & & 0.352 & 0.345 & 0.374 & 0.374 & 0.362 & 0.346 & 0.356 & 0.345 & 0.293 \\
    & F1.5 & & 0.398 & 0.384 & 0.402 & 0.393 & 0.378 & 0.351 & 0.360 & 0.342 & 0.274 \\ %old model
    & F2.0 & & 0.439 & 0.420 & 0.430 & 0.415 &  0.396 & 0.362 & 0.372 & 0.348 & 0.270 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS18}}} 
    & F0.5 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F1.0 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F1.5 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    & F2.0 & & nan &          nan &          nan &          nan &  nan &          nan &          nan &          nan &          nan \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{MO17}}} 
    & F0.5 & & 0.866 & 0.900 & 0.918 & 0.930 & 0.943 & 0.948 & 0.951 & 0.954 & 0.948 \\
    & F1.0 & & 0.907 & 0.928 & 0.936 & 0.941 & 0.944 & 0.942 & 0.938 & 0.932 & 0.902 \\
    & F1.5 & & 0.936 & 0.947 & 0.949 & 0.948 & 0.945 & 0.940 & 0.930 & 0.919 & 0.876 \\ %old model
    & F2.0 & & 0.954 & 0.959 & 0.957 & 0.953 &  0.946 & 0.939 & 0.926 & 0.913 & 0.862 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{PO18}}} 
    & F0.5 & & 0.610 & 0.630 & 0.639 & 0.647 & 0.664 & 0.656 & 0.663 & 0.657 & 0.651 \\
    & F1.0 & & 0.610 & 0.619 & 0.622 & 0.624 & 0.656 & 0.629 & 0.625 & 0.608 & 0.586 \\
    & F1.5 & & 0.622 & 0.623 & 0.623 & 0.620 & 0.660 & 0.623 & 0.612 & 0.589 & 0.559 \\ %old model
    & F2.0 & & 0.633 & 0.629 & 0.627 & 0.621 & 0.665 & 0.623 & 0.607 & 0.582 & 0.547 \\
    \bottomrule
\end{tabularx}

==> supplementary_data/multiclass_tversky_stderr.tex <==
% Results for new model:
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Type & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & 0.75/0.75 & 1.0/1.0\\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Dice}}} 
&All &        &        0.009 &        0.009 &        0.009 &        0.009 & 0.010 &        0.010 &        0.010 &        0.010 &        0.010 &        0.010 & 0.010 \\
&WT &        &        0.007 &        0.007 &        0.006 &        0.007 & 0.007 &        0.007 &        0.007 &        0.007 &        0.008 &        0.007 & 0.007 \\
&TC &        &        0.012 &        0.011 &        0.012 &        0.012 & 0.013 &        0.013 &        0.014 &        0.014 &        0.014 &        0.013 & 0.014 \\
&ET &        &        0.016 &        0.016 &        0.017 &        0.017 & 0.017 &        0.017 &        0.018 &        0.017 &        0.016 &        0.018 & 0.017 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{4}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
&All &        &        0.008 &        0.009 &        0.009 &        0.010 & 0.010 &        0.010 &        0.010 &        0.010 &        0.010 &        0.010 & 0.010 \\
&WT &        &        0.009 &        0.008 &        0.008 &        0.008 & 0.009 &        0.008 &        0.009 &        0.009 &        0.010 &        0.008 & 0.008 \\
&TC &        &        0.012 &        0.012 &        0.013 &        0.013 & 0.014 &        0.014 &        0.014 &        0.014 &        0.014 &        0.014 & 0.014 \\
&ET &        &        0.014 &        0.014 &        0.015 &        0.016 & 0.016 &        0.016 &        0.016 &        0.015 &        0.015 &        0.016 & 0.016 \\
    \bottomrule
\end{tabularx}

==> supplementary_data/tversky_fmeasures_stderr.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Measure & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & 0.75/0.75 & 1.0/1.0 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{BR18}}} 
    & F0.5 & & 0.008 & 0.007 & 0.007 & 0.007 & 0.006 & 0.005 & 0.006 & 0.006 & 0.006 &  0.006 & 0.007 \\
    & F1.0 & & 0.007 & 0.006 & 0.006 & 0.006 & 0.006 & 0.006 & 0.007 & 0.007 & 0.008 &  0.006 & 0.007 \\
    & F1.5 & & 0.006 & 0.005 & 0.006 & 0.006 & 0.006 & 0.006 & 0.007 & 0.008 & 0.009 &  0.007 & 0.007 \\
    & F2.0 & & 0.005 & 0.005 & 0.006 & 0.007 & 0.007 & 0.007 & 0.008 & 0.009 & 0.009 &  0.007 & 0.007 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS17}}} 
    & F0.5 & & 0.034 & 0.035 & 0.039 & 0.040 & 0.037 & 0.038 & 0.038 & 0.037 & 0.036 &  0.036 & 0.037 \\
    & F1.0 & & 0.036 & 0.035 & 0.037 & 0.037 & 0.034 & 0.034 & 0.033 & 0.034 & 0.031 &  0.033 & 0.035 \\
    & F1.5 & & 0.037 & 0.036 & 0.036 & 0.036 & 0.034 & 0.033 & 0.032 & 0.034 & 0.030 &  0.033 & 0.035 \\
    & F2.0 & & 0.039 & 0.037 & 0.036 & 0.037 & 0.034 & 0.034 & 0.032 & 0.035 & 0.030 &  0.034 & 0.036 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{IS18}}} 
    & F0.5 & & 0.024 & 0.026 & 0.026 & 0.027 & 0.028 & 0.028 & 0.029 & 0.029 & 0.030 &  0.028 & 0.028 \\
    & F1.0 & & 0.025 & 0.026 & 0.026 & 0.026 & 0.027 & 0.027 & 0.027 & 0.027 & 0.027 &  0.027 & 0.027 \\
    & F1.5 & & 0.025 & 0.026 & 0.026 & 0.026 & 0.027 & 0.027 & 0.027 & 0.026 & 0.026 &  0.027 & 0.027 \\
    & F2.0 & & 0.026 & 0.026 & 0.027 & 0.026 & 0.027 & 0.027 & 0.027 & 0.026 & 0.025 &  0.027 & 0.027 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{MO17}}} 
    & F0.5 & & 0.004 & 0.004 & 0.004 & 0.003 & 0.003 & 0.003 & 0.002 & 0.003 & 0.002 &  0.003 & 0.003 \\
    & F1.0 & & 0.003 & 0.003 & 0.003 & 0.003 & 0.003 & 0.003 & 0.002 & 0.003 & 0.003 &  0.002 & 0.003 \\
    & F1.5 & & 0.002 & 0.002 & 0.002 & 0.002 & 0.002 & 0.003 & 0.002 & 0.003 & 0.003 &  0.002 & 0.003 \\
    & F2.0 & & 0.002 & 0.002 & 0.002 & 0.002 & 0.002 & 0.003 & 0.002 & 0.003 & 0.004 &  0.002 & 0.003 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{PO18}}} 
    & F0.5 & & 0.009 & 0.009 & 0.009 & 0.009 & 0.009 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.009 \\
    & F1.0 & & 0.009 & 0.009 & 0.009 & 0.009 & 0.009 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 \\
    & F1.5 & & 0.009 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 \\
    & F2.0 & & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 & 0.010 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{WM17}}} 
    & F0.5 & & 0.019 & 0.019 & 0.018 & 0.020 & 0.018 & 0.019 & 0.017 & 0.018 & 0.020 &  0.020 & 0.019 \\
    & F1.0 & & 0.018 & 0.018 & 0.018 & 0.018 & 0.019 & 0.020 & 0.019 & 0.020 & 0.021 &  0.019 & 0.020 \\
    & F1.5 & & 0.018 & 0.019 & 0.018 & 0.019 & 0.020 & 0.021 & 0.020 & 0.021 & 0.021 &  0.019 & 0.021 \\
    & F2.0 & & 0.017 & 0.019 & 0.019 & 0.019 & 0.021 & 0.021 & 0.021 & 0.021 & 0.020 &  0.020 & 0.021 \\ 
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{WM17\textsuperscript{DM}}}} 
    & F0.5 & & 0.018 & 0.017 & 0.018 & 0.017 & 0.017 & 0.018 & 0.019 & 0.020 & 0.032 &  0.018 & 0.018 \\
    & F1.0 & & 0.018 & 0.018 & 0.018 & 0.018 & 0.019 & 0.020 & 0.022 & 0.023 & 0.030 &  0.020 & 0.020 \\
    & F1.5 & & 0.018 & 0.018 & 0.020 & 0.020 & 0.020 & 0.022 & 0.023 & 0.024 & 0.029 &  0.021 & 0.022 \\
    & F2.0 & & 0.018 & 0.019 & 0.021 & 0.021 & 0.021 & 0.022 & 0.024 & 0.024 & 0.028 &  0.022 & 0.023 \\
    \bottomrule
\end{tabularx}


==> supplementary_data/tversky_stderr.tex <==
\begin{tabularx}{\linewidth}{lsXYYYYYYYYY|YY}
    \toprule
    & Dataset & \multicolumn{1}{r}{\lapbox[\width]{1em}{\emph{$\alpha/\beta$} $\rightarrow$}} & 0.1/0.9 & 0.2/0.8 & 0.3/0.7 & 0.4/0.6 & 0.5/0.5 & 0.6/0.4 & 0.7/0.3 & 0.8/0.2 & 0.9/0.1 & 0.75/0.75 & 1.0/1.0 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Dice}}} 
    &BR18 &        &        0.007 &        0.006 &        0.006 &        0.006 & 0.006 &        0.006 &        0.007 &        0.007 &        0.008 &        0.006 & 0.007 \\
    &IS17 &        &        0.036 &        0.035 &        0.037 &        0.037 & 0.034 &        0.034 &        0.033 &        0.034 &        0.031 &        0.033 & 0.035 \\
    &IS18 &        &        0.025 &        0.026 &        0.026 &        0.026 & 0.027 &        0.027 &        0.027 &        0.027 &        0.027 &        0.027 & 0.027 \\
    &MO18 &        &        0.003 &        0.003 &        0.003 &        0.003 & 0.003 &        0.003 &        0.002 &        0.003 &        0.003 &        0.002 & 0.003 \\
    &PO18 &        &        0.009 &        0.009 &        0.009 &        0.009 & 0.009 &        0.010 &        0.010 &        0.010 &        0.010 &          0.010 & 0.010 \\
    &WM17 &        &        0.018 &        0.018 &        0.018 &        0.018 & 0.019 &        0.020 &        0.019 &        0.020 &        0.021 &        0.019 & 0.020 \\
    &WM17\textsuperscript{DM} &        &        0.018 &        0.018 &        0.018 &        0.018 & 0.019 &        0.020 &        0.022 &        0.023 &        0.030 &        0.020 & 0.020 \\
    \midrule
    \parbox[t]{7mm}{\centering\multirow{5}{*}{\rotatebox[origin=c]{90}{Jaccard}}}
    &BR18 &        &        0.008 &        0.007 &        0.008 &        0.008 & 0.008 &        0.007 &        0.008 &        0.009 &        0.010 &        0.008 & 0.008 \\
    &IS17 &        &        0.028 &        0.027 &        0.028 &        0.029 & 0.027 &        0.026 &        0.025 &        0.025 &        0.022 &        0.026 & 0.028 \\
    &IS18 &        &        0.022 &        0.023 &        0.023 &        0.023 & 0.023 &        0.023 &        0.023 &        0.023 &        0.022 &        0.024 & 0.024 \\
    &MO18 &        &        0.004 &        0.004 &        0.004 &        0.004 & 0.004 &        0.004 &        0.003 &        0.004 &        0.004 &        0.003 & 0.004 \\
    &PO18 &        &        0.008 &        0.009 &        0.009 &        0.009 & 0.009 &        0.009 &        0.009 &        0.009 &        0.009 &          0.009 & 0.009 \\
    &WM17 &        &        0.017 &        0.019 &        0.019 &        0.021 & 0.021 &        0.021 &        0.021 &        0.021 &        0.019 &        0.021 & 0.022 \\
    &WM17\textsuperscript{DM} &        &        0.017 &        0.018 &        0.020 &        0.021 & 0.021 &        0.022 &        0.023 &        0.023 &        0.026 &        0.022 & 0.022 \\
    \bottomrule
\end{tabularx}
